Genus expansion for non-linear random matrix ensembles with applications to neural networks

We present a unified approach to studying certain non-linear random matrix ensembles and associated random neural networks at initialization. This begins with a novel series expansion for neural networks which generalizes Fa\'a di Bruno's formula to an arbitrary number of compositions. The role of monomials is played by random multilinear maps indexed by directed graphs, whose edges correspond to random matrices. Crucially, this expansion linearizes the effect of the activation functions, allowing for the direct application of Wick's principle and the genus expansion technique. As an application, we prove several results about neural networks with random weights. We first give a new proof of the fact that they converge to Gaussian processes as their width tends to infinity. Secondly, we quantify the rate of convergence of the Neural Tangent Kernel to its deterministic limit in Frobenius norm. Finally, we compute the moments of the limiting spectral distribution of the Jacobian (only the first two of which were previously known), expressing them as sums over non-crossing partitions. All of these results are then generalised to the case of neural networks with sparse and non-Gaussian weights, under moment assumptions.

==> Sections/GPlimit.tex <==
We start by considering the distributional limit of feed-forward networks, recovering a result of \cite{matthews2018gaussian}. 

\begin{assumption}\label{assumption:GP_lim}
    Assume that the input dimension $N_0$ of $\Phi_L$ is be fixed, and that $N_{\ell}=N$ for all other layers $\ell > 0$.
\end{assumption}

\begin{theorem}[Gaussian process limit of neural networks]\label{thm:GPlimit}
    Assume that $\sigma_0=1$ and $\sigma_{\ell} = N_{\ell}^{-1/2}$  for $\ell\geq 1$ then for any $M,L \geq 1$ we have 
    \begin{equation}\label{eqn:GP_limit}
        ([\Phi_{L}]_1,...,[\Phi_{L}]_M) \xrightarrow[N \to \infty]{d} \mathcal{GP}(0,K_{L} \otimes \mathbf{I}_M)
    \end{equation}
    where the right hand side is a Gaussian Process indexed on $\bR^{N_0}$, with diagonal covariance function defined by
        \begin{gather*}
        K_{0}(\bx,\by) = \sprod{\bx}{\by}_{\bR^{N_0}}, ~
        K_{\ell+1}(\bx,\by) = \E\left[ \varphi_{\ell+1}(X_{\ell}) \varphi_{\ell+1}(Y_{\ell}) \right] \\
        (X_{\ell},Y_{\ell}) \sim \mathcal{N}\left(0,
        \begin{bmatrix}
            K_{\ell}(\bx,\bx) & K_{\ell}(\bx,\by)
            \\
            K_{\ell}(\by,\bx) & K_{\ell}(\by,\by)
        \end{bmatrix}\right).
    \end{gather*}
\end{theorem}

\subsubsection{From operators to graphs:}
Following the pipeline above, we begin by considering the coordinate-wise tree expansion of $\Phi_{L}$ given in equation \ref{eqn:tree_exp_coords}:
\[
[\Phi_{L}(\bx)]_k = \sum_{\tau \in \mathbb{T}_{L,k}} \frac{\varphi_{\tau}}{s(\tau)} \bW_{\tau} \bx_\tau  \in \bR.
\]

\subsubsection{Graph scaling limits:}
\tieBreaker{For Prof. Bin Salvi: subsubsection headers yes or no?}
To find the distributional limit of $[\Phi_{L}(\bx)]_k$ using this expansion, we thus need a limit for the joint distribution of $(\bW_{\tau} ~|~ \tau \in \mathbb{T}_{L,k})$ as $N \to \infty$. Note that we have not made any assumptions on the variances $\sigma_{\ell}^2$ yet: as will soon become apparent, only one such choice yields a canonically meaningful result, and it will correspond to the so-called ``GP limit" initialization {\color{orange} (see, e.g. \cite{})}. 

We compute the mixed moments of the $\bW_{\tau}$ using Proposition \ref{prop:mixedmoments_}, which yields
\begin{align}\label{eq:mixedmoments}
    \E\bigg\{\prod_{i=1}^{m}\big(\bW_{\tau_i}-\sum_{\phi\in \mathcal{P}_{\mathrm{A}}(G_i)}\mathbf{W}_{(G_i)_{\phi}}\big)\bigg\}=\sum_{\phi \in \mathcal{P}_{\mathrm{AF}}(G)} \mathbf{W}_{G_{\phi}}.
\end{align}
To identify the leading terms on the right hand side, we must therefore identify the pairings $\phi\in \mathcal{P}_{\mathrm{AF}}(G)$ which maximize $\mathbf{W}_{G_\phi}$, and the following lemma shows that these precisely those in $\mathcal{P}_{\mathrm{bi}}(G)$.

\begin{lemma}\label{lemma:GP_scaling}
    Under assumption \ref{assumption:GP_lim}, for any $L \geq 0$, $i = 1, \dots, m$ and $1 \leq k_i \leq N_{L + 1}$ let $\tau_i \in \bT_{L,k_i}$. Then 
    \begin{equation}
    \sum_{\psi \in \mathcal{P}_{\mathrm{A}}(\tau_i)} \mathbf{W}_{(\tau_i)_{\psi}}
    = 0,
    \end{equation} 
    \begin{equation}
        \sum_{\phi \in \mathcal{P}_{\mathrm{AF}}(\sqcup_i \tau_i)} \mathbf{W}_{(\sqcup_i \tau_i)_{\phi}}
        = N^{{\tfrac{1}{2}|E(\sqcup_i \tau_i)| - |\mathcal{L}(\sqcup_i \tau_i)}|}\left(\alpha_{\sqcup_i \tau_i} + \mathcal{O}\Big(\frac{1}{N}\Big)\right).
    \end{equation}
    where $\mathcal{L}(\sqcup_i\tau_i)$ denotes the set of \textit{leaves} of $\sqcup_i\tau_i$ (endpoints of $0$-labeled edges).
\end{lemma}
Applying this lemma to (\ref{eq:mixedmoments}) gives
\begin{equation}\label{eqn:GP_tree_scaling}
     \E\left\{\prod_{i=1}^{m} \bW_{\tau_i}\right\}
     = \sigma_{\sqcup_i \tau_i} N^{\tfrac{1}{2}({|E(\sqcup_i \tau_i)| - \mathcal{L}(\sqcup_i \tau_i)})}
        \left(\alpha_{\sqcup_i \tau_i} + \mathcal{O}\Big(\frac{1}{N}\Big)\right).
\end{equation}
If we want to have a well-defined distributional limit for $[\Phi_{L}(x)]_k$, we must thus choose the standard deviations $\sigma_{\ell}$ so that the above quantity is $\mathcal{O}(1)$ for all choices $\tau_i \in \bT_{L,k_i}$. This is equivalent to requiring that
$\sigma_{\tau} N^{\tfrac{1}{2}({|E(\tau)| - \mathcal{L}(\tau)})} = \mathcal{O}(1)$ for all $L \geq 1$ and $\tau \in \mathbb{T}_{L,k}$, which is in turn equivalent to 
\[
 \sigma_0=\mathcal{O}(1) \text{ and } \sigma_{\ell} = \mathcal{O}(N_{\ell}^{-1/2}) \,\,  \forall \ell \geq 1.
\]
The canonical choice would then be the one for which $\sigma_{\tau} N^{\tfrac{1}{2}({|E(\tau)| - \mathcal{L}(\tau)})} = 1$: this is exactly the ``GP limit" parametrization of Neural Networks (see \cite{}), under which the method of moments then gives the following limit.
\begin{proposition}\label{lemma:joint_limit_trees}
    Under assumption \ref{assumption:GP_lim}, let $\sigma_0=1$ and $\sigma_{\ell} = N_{\ell}^{-1/2}$  for $\ell\geq 1$.
    Then for any $M,L \geq 1$  we have 
    \begin{equation}
        \left(\bW_{\tau} ~\bigg|~ \tau \in \bigcup_{k=1}^M \mathbb{T}_{L,k}\right) 
        \xrightarrow[N \to \infty]{d} 
        \left(Z_{\tau} ~\bigg|~ \tau \in \bigcup_{k=1}^M \mathbb{T}_{L,k}\right) 
        \sim \mathcal{GP}(0,C)
    \end{equation}
    with the Gaussian Process indexed on $\bigcup_{k=1}^M \mathbb{T}_{L,k}$ having covariance $C(\tau,\eta) = \alpha_{\tau \sqcup \eta}$.
\end{proposition}

\subsubsection{Combinatorics of the Limits:}
We can make the previous result more precise by analyzing the combinatorial structure of the limiting covariances $\alpha_{\tau\sqcup\eta}$. This is achieved by the following lemma proved in Section \ref{sec:extensions}.
\begin{lemma}\label{lemma:alpha_trees}
    Given $\tau = [\tau_1 \cdots \tau_M]_{\ell + 1}, \eta = [\eta_1 \cdots \eta_{M'}]_{\ell + 1}\in \bT_{\ell,i}$ we can write
      \[
    \alpha_{\tau\sqcup\eta} = \sum_{\pi} \prod_{\{\beta, \tilde \beta\} \in \pi} \alpha_{\beta \sqcup \tilde\beta}
    \]
    where the sum is over all pairings $\pi$ of the elements of $(\tau_1, \dots, \tau_M, \eta_1, \dots, \eta_{M'})$.
\end{lemma}

\subsubsection{Back to analysis:}
We are now ready to prove theorem \ref{thm:GPlimit}.
\begin{proof}[Proof of theorem \ref{thm:GPlimit}]
    It follows directly from proposition \ref{lemma:joint_limit_trees} and lemma \ref{lemma:alpha_trees} that 
    \[
        ([\Phi_\ell]_1,...,[\Phi_\ell]_{M})\overset{d}{\longrightarrow}\mathcal{GP}(0, K_\ell\otimes \mathbf{I}_M)
    \]
    where $K_{\ell}$ is defined by
    \begin{equation}\label{eqn:GP_lim_tree}
        K_{\ell}(\bx,\by) = \sum_{\tau,\eta \in \bT_{\ell,1} } \frac{\varphi_{\tau}\varphi_{\eta}}{s(\tau) s(\eta)}\alpha_{\tau \sqcup \eta} \bx^{\tau} \by^{\eta} \in \bR.
    \end{equation}
    What's left is to show that this definition of $K_{\ell}$ coincides with the one in the theorem statement. We proceed by induction on $\ell$, the base case being true by definition. The inductive step follows by applying Proposition \ref{app:prop:expectation_tree_expansion} with $\cA = \bT_{\ell,1}$ and $\lambda_{\tau,\eta} = \frac{\varphi_{\tau}\varphi_{\eta}}{s(\tau) s(\eta)}\alpha_{\tau \sqcup \eta}$.
    Recall that $\bT_{\ell+1,1}$ and $\bX_\cA$ are in bijection via $\tau := [\tau_1 \cdots \tau_m]_{\ell+1} \mapsto \bar\tau := \llbracket \tau_1 \cdots \tau_m \rrbracket$ and under this identification we have $s(\tau) = {\fs(\bar\tau)} \prod_i s(\tau_i)$, $\varphi_\tau = {
    (\varphi_{\ell+1})_{\bar\tau}} \prod_i \varphi_{\tau_i}$ and Lemma \ref{lemma:alpha_trees} gives 
    \[
    \alpha_{\tau\sqcup\eta} = \sum_{\pi \in \cP(\bar\tau \sqcup \bar\eta)} \prod_{\{\pi_1, \pi_2\} \in \pi} \alpha_{\pi_1 \sqcup \pi_2}.
    \]
\end{proof}


==> Sections/combinatorics-section.tex <==



% Our main task, which is achieved by theorem \ref{thm:aformula}, will be to count the number of acyclic edge pairings of decorated cycles. Recall that by an acyclic pairing $\phi$, we mean that the graph obtained by identifying edges paired by $\phi$ contains no (undirected) cycle. 
\subsection{The structure of acyclic edge pairings in decorated cycles}

Consider a $k-$tuple $\boldsymbol{\ell}=(\ell_1,...,\ell_k)$ of integers in $\mathbb{Z}_{\geq 1}$. Let $L:=\max_i \ell_i$, $m=\#\{i:\ell_i=L\}$, and $G(\boldsymbol{\tau},\boldsymbol{\eta})\in \mathrm{DC}(\boldsymbol{\ell})$. Recall that for each $i$, the vertex of $C(\boldsymbol{\tau},\boldsymbol{\eta})$ at which $\eta_{\ell_i}^{(i)}\circ\tau_{\ell_i}^{(i)}$ is rooted is labeled by $v_{i}$, and is the source of two $\ell_i$-labeled edges. Then any acyclic pairing $\phi \in \mathcal{P}(G(\boldsymbol{\tau},\boldsymbol{\eta}))$  admits the following decomposition.

\begin{lemma}\label{lem:firstdecomp}
    If $\phi \in\mathcal{P}(G(\boldsymbol{\tau},\boldsymbol{\eta}))$ is acyclic, then $\phi=\phi_C \sqcup \phi_{G\setminus C}$ for some $\phi_C\in\mathcal{P}(C(\boldsymbol{\tau},\boldsymbol{\eta}))$. In particular, all of the $L$-labeled edges of $C(\boldsymbol{\tau},\boldsymbol{\eta})$ are paired between themselves by some pairing $\phi_L\subseteq \phi_C$.
\end{lemma}
\begin{proof}
For $\phi$ to be acyclic, it must collapse the undirected cycle $C(\boldsymbol{\tau},\boldsymbol{\eta})$ and not create any new cycles in doing so. But this is only possible if edges of $C(\boldsymbol{\tau},\boldsymbol{\eta})$ are paired between themselves, as any edge that isn't paired this way would end up in a cycle (as depicted in figure \ref{fig:cyclicpairing} below).
\NicoComm{Is this enough to convey the proof?}
\begin{figure}[h]
    \centering
    \input{Figures/treecyclepairing}
    \caption{A cycle formed by pairing edges that belong to $C(\boldsymbol{\tau},\boldsymbol{\eta})$ with edges that do not.}
    \label{fig:cyclicpairing}
\end{figure}

Further, since edges can only be paired with other edges of the same label, $\phi$ must contain a pairing $\phi_{L}$ of the edges labeled by $L$ in $C(\boldsymbol{\tau},\boldsymbol{\eta})$.
\end{proof}

Let $\phi\in \mathcal{P}(G(\boldsymbol{\tau},\boldsymbol{\eta}))$ be acyclic, and $\phi_L$ be as in the lemma above. Now recall that each pair of adjacent, $L$-labeled edges in $C(\boldsymbol{\tau},\boldsymbol{\eta})$ shares a vertex $v_i$ for some unique $i\in\{1,...,k\}$. These $m$ pairs of $L$-labeled edges are thus in bijection with subsets
\NicoComm{Should we be more detailed?}
$v_{i_1},...,v_{i_m}$ of the vertices $v_1,...,v_k$. Through this bijection, $\phi_L\subseteq \phi$ induces a unique partition $\pi$ of $\{i_1,...,i_m\}$ (equivalently, of $\{1,...,m\}$), defined by letting $i_a$ and $i_b$ be in the same block of $\pi$ if they label endpoints of edges which have been paired by $\phi_{L}$. This is depicted in figure \ref{fig:noncrossingpartition}, and we write $\phi_L\sim \pi$ to denote the fact that $\phi_L$ induces $\pi$.
 \begin{figure}[ht]
    \centering
    \scalebox{.90}{\input{Figures/noncrossingdual}}
    \caption{A pairing $\phi_L$ of the $L$-labeled edges of a cycle $C(\boldsymbol{\tau},\boldsymbol{\eta})$ (left), the partition $\pi\in \mathrm{NC}(\{2,3,6,8\})$($\simeq \mathrm{NC}_4$) that is induced by $\phi_L$ (center), and $\pi$'s dual in $\{1,...,8\}$ (right). Here, $m=4$ and $k=8$.}
    \label{fig:noncrossingpartition}
\end{figure}

For acyclic $\phi$, it turns out that the partitions $\pi$ that arise this way must be non-crossing.

\begin{lemma} Let $\phi\in {G}(\boldsymbol{\tau},\boldsymbol{\eta})$ be acyclic, and $\phi_L\subset \phi$ be the pairing of $L$-labeled edges of $C(\boldsymbol{\eta},\boldsymbol{\tau})$ given by lemma \ref{lem:firstdecomp}. Then $\phi_L\sim \pi$ for some $\pi\in \mathrm{NC}_m$.
\end{lemma}
\NicoComm{Proof?}

\begin{remark}
    This corresponds to condition 2.4.1. (i) in \cite{dubach2021words}, our $C(\boldsymbol{\tau},\boldsymbol{\eta})$ playing the role of their polygon $f_w$.
\end{remark}
Indeed, if $\phi_L\sim \pi$ and $\pi$ admits a crossing, then a cycle is formed as depicted in figure \ref{fig:crossing} below. 
\NicoComm{Do these arguments suffice? could they be taken as hasty generalizations?}
Next, recall that by definition, $v_{i_a}$ is the root of $\eta_{L}^{(i_a)}\circ\tau_{L}^{(i_a)}$ for every $a\in \{1,...,m\}$. Upon identifying $L$-labeled edges of $C(\boldsymbol{\tau},\boldsymbol{\eta})$ by $\phi_L$, such trees get joined at their roots. More precisely, if $\phi_L\sim \pi$, then for every block $B=\{j_1,...,j_l\}$ of $\pi$ we obtain the tree $$(\tau^{(j_1)}_{L}\circ\eta^{(j_1)}_{L}\circ \cdots \circ  \tau^{(j_l)}_{L}\circ\eta^{(j_l)}_{L}):=\circ_{i=1}^l(\tau^{(j_i)}_{L}\circ\eta^{(j_i)}_{L}).$$
For $\phi$ to be acyclic, it must at the very least pair edges of such trees internally within each tree (otherwise, a cycle would be formed at their roots). We therefore get, for each block $B=\{j_1,..,j_l\}$ of $\pi$, an acyclic pairing $\phi_B\in \mathcal{P}(\circ_{i=1}^l(\tau_{L}^{(j_i)}\circ\eta_{L}^{j_i}))$. 
    \begin{figure}[ht]
    \centering
    \input{Figures/crossingpartition}
    \caption{If $\phi_L\sim \pi$ and $\pi$ has a crossing, then identifying edges according to $\phi_L$ creates a cycle.}
    \label{fig:crossing}
\end{figure}



Having now paired $L$--labeled edges belonging to $C(\boldsymbol{\tau},\boldsymbol{\eta})$ (using $\phi_L$), and those belonging to trees of height $L$ decorating this cycle (using the $\phi_B$'s), we must describe how $\phi$ pairs the remaining edges. Crucially, observe that the unpaired edges are labeled only from $\{1,...,L-1\}$ and form disjoint decorated cycles themselves. To be precise, we will need the following definition.

\begin{definition}
    Let $G(\boldsymbol{\tau},\boldsymbol{\eta})\in \mathrm{DC}(\boldsymbol{\ell}), \phi_L$ be as above and $\phi_L\sim \pi$ for some $\pi\in \mathrm{NC}_m$. 
    Let $\tilde{B}$ be a block of a $\pi_k^*\in\mathrm{NC}_k$, recalling that $k=|\boldsymbol{\ell}|$. 
    Then the \textup{restriction of $G(\boldsymbol{\tau},\boldsymbol{\eta})_{\phi_L}$ to $\tilde{B}$} is the decorated cycle determined by the trees
    \begin{align*}
        (\boldsymbol{\tau},\boldsymbol{\eta})\big|_{\tilde{B}}=\big((\tau^{(b)}_{j})_{j=1}^{h}, (\eta_j^{(b)})_{j=1}^h\big)_{b\in \tilde{B}},\quad h= \begin{cases}
            \ell_b \mbox{ if $\ell_b \neq L$} \\
            \ell_b-1 \mbox{ if $\ell_b = L$} \\
        \end{cases}
    \end{align*}
    and whose distinguished vertices $\{v'_b\}_{b\in B}$ are the roots of $\tau^{(b)}_h\circ\eta^{(b)}_h $for each $b\in \tilde{B}$.
\end{definition}
\begin{remark}
      $G(\boldsymbol{\tau},\boldsymbol{\eta})\big|_{\tilde{B}}$ is an element of $\mathrm{DC}({\hat{\boldsymbol{{\ell}}}_{\tilde{B}}})$, where $\boldsymbol{\ell}_{\tilde{B}}$ is the cycle of $\pi_k^*(\boldsymbol{\ell})$ corresponding to the block $\tilde{B}$. For instance, let $k=4$, $\ell=(2,3,2,1)$, and $\pi_k^*=\{B_1,B_2\}=\{\{1,2\},\{3,4\}\}$. Then $\hat{\boldsymbol{\ell}}=(2,2,2,1)$, $\pi_k^*(\boldsymbol{\ell})=(2,2)(2,1)$ and $\hat{\boldsymbol{\ell}}_{B_1}=(2,2)$.
\end{remark}
Returning to our previous point, the leftover edges (that were not paired by $\phi_L$ or $\phi_B$) form one decorated cycle per block of $\pi_k^*$, which are given by
\[
    G(\boldsymbol{\tau},\boldsymbol{\eta})\big|_{\tilde{B}},\quad \tilde{B}\in \pi_*^k.
\]
For $\phi$ to be acyclic, we claim that the edges of each of these $G(\boldsymbol{\tau},\boldsymbol{\eta})\big|_{\tilde{B}}$ must once again be paired internally. This is because the $G(\boldsymbol{\tau},\boldsymbol{\eta})\big|_{\tilde{B}}$ are connected to one another in $G(\boldsymbol{\tau},\boldsymbol{\eta})_{\phi_L, \{\phi_B\}_{B\in \pi}}$ by paths whose edges that have already been paired by $\phi_B$ or $\phi_L$; pairing some $e\in G(\boldsymbol{\tau},\boldsymbol{\eta})\big|_{\tilde{B}}$ to another $e'\in G(\boldsymbol{\tau},\boldsymbol{\eta})\big|_{\tilde{B'}}$ would then create a cycle which we cannot collapse (as in figure \ref{fig:crossing}). Put differently, this implies that any pairing $\phi'$ of the remaining edges can be decomposed into a disjoint union as follows:
\[ 
    {\phi'}=\bigsqcup_{\tilde{B}\in \pi_k^*} \phi'_{\tilde{B}}.
\]
Summarizing everything we have said so far, an acyclic pairing $\phi\in \mathcal{P}(G(\boldsymbol{\tau},\boldsymbol{\eta}))$ consists of the following. 
\begin{enumerate}
    \item A pairing $\phi_L$ of the $L$-labeled edges of $C(\boldsymbol{\tau},\boldsymbol{\eta})$, such that $\phi_L\sim \pi\in \mathrm{NC}_m$.
    \item For every block $B=\{j_1,...,j_l\}$ of $\pi$, a pairing in $\mathcal{P}(\circ_{i=1}^l(\tau_L^{(j_i)}\circ\eta_L^{(j_i)})$ which is acyclic.
    \item For every block $\tilde{B}=\{b_1,...,b_l\}$ of $\pi^*_k$, a pairing $\phi_{\tilde{B}}\in \mathcal{P}(G(\boldsymbol{\tau},\boldsymbol{\eta}))\big|_{\tilde{B}}$.
\end{enumerate}
Recalling that $a_{G}$ denotes the number of acyclic pairings in $\mathcal{P}(G)$ for any graph $G$, the above is equivalent the following theorem.
\begin{theorem}
    [Define everything here]
    \[
        a_{G(\boldsymbol{\tau},\boldsymbol{\eta})}=\sum_{\pi \in \mathrm{NC}_m} \left(\prod_{B\in \pi}a_{\circ_{i=1}^l(\tau_{L}^{(j_i)}\circ\eta_{L}^{(j_i)})}\right)\left(\prod_{\tilde{B}\in \pi^*_k}a_{G(\boldsymbol{\tau},\boldsymbol{\eta})\big|_{\tilde{B}}}\right)
    \]
\end{theorem}
An example is in order to help elucidate this theorem and the heavy notation we have introduced. Consider the tuple $\boldsymbol{\ell}=(2,1,2,2)$, in which case $k=4$, $m=3$, and $L=2$. Using the same notation as above, let $G(\boldsymbol{\tau},\boldsymbol{\eta})\in \mathrm{DC}(\boldsymbol{\ell})$, and consider a pairing $\phi_2$ of the $2$-labeled edges of $C(\boldsymbol{\tau},\boldsymbol{\eta})$ satisfying $\phi_2 \sim \pi = \{\{1,3,4\}\}$.
This partition $\pi$ is depicted in figure \ref{fig:fullexamplepartition}, alongside its dual $\pi_4^*$ (relative to $\{1,2,3,4\}$).

\begin{figure}[ht]
    \centering
     \scalebox{.8}{\input{Figures/fullexamplepartition}}
        \caption{A partition $\pi=\{\{1,3,4\}\}\in \mathrm{NC}(\{1,3,4\})$ and its dual $\pi_4^*$.}
    \label{fig:fullexamplepartition}
\end{figure}


For this setup, the decomposition outlined above is depicted in full detail in the following figure.
\begin{figure}[ht]
    \centering
         \scalebox{.85}{\input{Figures/fullexample}}
    \caption{The partition $\pi$ only has one block, which gives rise to the tree $\eta_2^{(1)}\circ\tau_2^{(1)}\circ \eta_2^{(3)}\circ\tau_2^{(3)}\circ\eta_2^{(4)}\circ\tau_2^{(4)}$. Its dual has three blocks, giving rise to three decorated cycles: $G(\boldsymbol{\tau},\boldsymbol{\eta})\big|_{\{1,4\}}\in \mathrm{DC}((1,1))$, $G(\boldsymbol{\tau},\boldsymbol{\eta})\big|_{\{2\}}\in \mathrm{DC}((1))$ and $G(\boldsymbol{\tau},\boldsymbol{\eta})\big|_{\{3\}}\in \mathrm{DC}((1))$.}
    \label{fig:fullexample}
\end{figure}


==> Sections/dump.tex <==


% \subsection{Counting acyclic pairings of decorated cycles}
% For our analysis, we wish to evaluate weighted sums of the form 
% \[
%     \sum_{G\in \mathcal{G}} w_G\cdot a_G,
% \]
% where $\mathcal{G}$ is a set of graphs and $w_G\in \mathbb{Z}$ is some weight. For instance, to study the spectrum of the input-output Jacobian of feed-forward networks, $\mathcal{G}$ will be $\mathrm{DC}(\boldsymbol{\ell})$ and 
% \[
%     w_G = \prod_\tau \frac{\varphi_\tau\gamma_\tau}{\sigma(\tau)}, 
% \]
% where $\varphi_\tau, \gamma_\tau, \sigma_\tau$ are as defined in \ref{}, and the product is taken over all trees rooted at vertices belonging to the unique cycle of $G$. These choices of $\mathcal{G}$ and $w_G$ gives rise to the quantity
% \[
%     \mathrm{M}(\boldsymbol{\ell}) = \sum_{G\in \mathrm{DC}(\boldsymbol{\ell})} w_G\cdot a_G,
% \]
% for which theorem \ref{thm:Mrecursion} gives a recursive formula. We extend $\mathrm{M}$ to all elements of the symmetric group $S_k$ by defining  to be multiplicative over cycles (i.e. $\mathrm{M}(\boldsymbol{\ell}\bf{m}):=\mathrm{M}(\boldsymbol{\ell})\mathrm{M}(\bf{m})$). Lastly, we define 
% \[
%     \mu_{k, L} := \sum_{\tau_1, \dots, \tau_{2k} \in \bT_{L}} \left( \prod_i \frac{\varphi_{\tau_i} \gamma_{\tau_i}} {\sigma(\tau_i)}\right)
%     a_{\circ_i \tau_i},
% \]
% where $\circ_i \tau_i$ is the tree obtained by attaching $\tau_1,...,\tau_{2k}$ by their root vertex. If $\pi=\{B_1,...,B_j\}$, we write $\mu_{\pi, L}$ to mean $\prod_i \mu_{|B_i|, L}$.

% We are now ready to state our main result.
% \begin{theorem}[Recursive formula for $\mathrm{M}$]\label{thm:Mrecursion}
% For any $k-$tuple $\boldsymbol{\ell}=(\ell_1,...,\ell_k)$ of integers in $\mathbb{Z}_{\geq 1}$, let $L:=\max_i \ell_i$ and $m:= \#\{i:\ell_i=L\}$. Then
% \begin{equation}
%     \mathrm{M}(\boldsymbol{\ell})= \sum_{\substack{\pi\in \mathrm{NC}_m}} \mu_{\pi, L} \mathrm{M}(\pi^*_k(\hat{\boldsymbol{\ell}}))
% \end{equation}
% \end{theorem}
% It is clear that enumerating the graphs in $\mathrm{DC}(\boldsymbol{\ell})$ is equivalent to enumerating all possible choices of trees $\tau_{j}^{(i)},\eta_{j}^{(i)}$ where $i=1,...,k$, $j=1,...,\ell_i$ and $\tau_j^{(i)}\in \bT_{j}$. Letting $$(\boldsymbol{\tau},\boldsymbol{\eta})=(\tau_{j}^{(i)}, \eta_{j}^{(i)})_{i,j}\in \prod_{i=1}^k (\bT_{\ell_i}\times\cdots\times \bT_{1})$$ denote one such choice and $G(\boldsymbol{\tau},\boldsymbol{\eta})$ denote its corresponding decorated cycle, we can therefore express $\mathrm{M}(\boldsymbol{\ell})$ as a sum over all $(\boldsymbol{\tau},\boldsymbol{\eta})$ by writing
% \[
%     \mathrm{M}(\boldsymbol{\ell}) = \sum_{(\boldsymbol{\tau},\boldsymbol{\eta})} w_{(\boldsymbol{\tau},\boldsymbol{\eta})}a_{G(\boldsymbol{\tau},\boldsymbol{\eta})},
% \]
% where 
% \[
%     w_{(\boldsymbol{\tau},\boldsymbol{\eta})} = \prod_{i=1}^{k}\prod_{j=1}^{\ell_i}\frac{\varphi_{\tau_j^{(i)}}\varphi_{\eta_j^{(i)}}}{\sigma\big(\tau_j^{(i)}\big)\eta\big(\tau_j^{(i)}\big)}\gamma_{\tau_j^{(i)}}\gamma_{\eta_j^{(i)}}.
% \]
% Note that each $G(\boldsymbol{\tau},\boldsymbol{\eta})$ is, by definition, comprised of a cycle of length $2\sum_{i}\ell_i$, to which the roots of  $(\boldsymbol{\tau},\boldsymbol{\eta})$ belong. We refer to this cycle as $C(\boldsymbol{\tau},\boldsymbol{\eta})$ in what follows, and let $v_{i}$ denote the vertex of $C(\boldsymbol{\tau},\boldsymbol{\eta})$ at which $\eta_{\ell_i}^{(i)}$ and $\tau_{\ell_i}^{(i)}$ are rooted (for each $i$, $v_i$ is thus the source of two $\ell_i$-labeled edges).

% To prove the theorem, we analyze the structure of acyclic pairings of edges of $G(\boldsymbol{\tau}, \boldsymbol{\eta})$ in order to evaluate $a_{G(\boldsymbol{\tau}, \boldsymbol{\eta})}$. We begin with the following decomposition.

% \begin{lemma}\label{lem:firstdecomp}
%     If $\phi \in\mathcal{P}(G(\boldsymbol{\tau},\boldsymbol{\eta}))$ is acyclic, then $\phi=\phi_C \sqcup \phi_{G\setminus C}$ for some $\phi_C\in\mathcal{P}(C(\boldsymbol{\tau},\boldsymbol{\eta}))$. In particular, all of the $L$-labeled edges of $C(\boldsymbol{\tau},\boldsymbol{\eta})$ are paired between themselves by some pairing $\phi_L\subseteq \phi_C$.
% \end{lemma}
% \begin{proof}
% Observe that if an edge of $C(\boldsymbol{\tau},\boldsymbol{\eta})$ is paired to an edge outside of this cycle, then $G(\boldsymbol{\tau},\boldsymbol{\eta})_{\phi}$ (the graph obtained from $G(\boldsymbol{\tau},\boldsymbol{\eta})$ after identifying edges paired by $\phi$) will contain a cycle. It follows that for $\phi$ to be acyclic, all edges in $C(\boldsymbol{\tau},\boldsymbol{\eta})$ must be paired within themselves. Further, since edges can only be paired with other edges of the same label, $\phi$ must contain a pairing $\phi_{L}$ of the edges labeled by $L$ in $C(\boldsymbol{\tau},\boldsymbol{\eta})$.
% \end{proof}

% Let $\phi\in \mathcal{P}(G(\boldsymbol{\tau},\boldsymbol{\eta}))$ be acyclic, and $\phi_L$ be as in the lemma above. Now recall that each pair of adjacent, $L$-labeled edges in $C(\boldsymbol{\tau},\boldsymbol{\eta})$ shares a vertex $v_i$ for some unique $i\in\{1,...,k\}$. In other words, these $m$ pairs of $L$-labeled edges are in bijection with a subset $v_{i_1},...,v_{i_m}$ of the vertices $v_1,...,v_k$. Through this bijection, $\phi_L\subseteq \phi$ induces a unique partition $\pi$ of $\{i_1,...,i_m\}$ (equivalently, of $\{1,...,m\}$), defined by letting $i_a$ and $i_b$ be in the same block of $\pi$ if they label endpoints of edges which have been paired by $\phi_{L}$. This is depicted in figure \ref{fig:noncrossingpartition}, and we write $\phi_L\sim \pi$ to denote the fact that $\phi_L$ induces $\pi$.

% It turns out that the partitions $\pi$ that arise this way must be non-crossing.

% % It turns out that pairings acyclic pairing $\phi$ which do not lead to the creation of a cycle in $G(\boldsymbol{\tau},\boldsymbol{\eta})$ have admit a very specific structure, which is revealed by the partition of $\{1,...,m\}$ that they induce. 
%  \begin{figure}
%     \centering
%     \include{Figures/noncrossingdual}
%     \caption{Caption}
%     \label{fig:noncrossingpartition}
% \end{figure}

% \begin{lemma} Let $\phi\in {G}(\boldsymbol{\tau},\boldsymbol{\eta})$ be acyclic, and $\phi_L\subset \phi$ be the pairing of $L$-labeled edges of $C(\boldsymbol{\eta},\boldsymbol{\tau})$ given by lemma \ref{lem:firstdecomp}. Then $\phi_L\sim \pi$ for some $\pi\in \mathrm{NC}_m$.
%  \end{lemma}
% \begin{proof}
%     See the following section.
% \end{proof}

% Recall that by definition, $v_{i_a}$ is the root of $\eta_{L}^{(i_a)}\circ\tau_{L}^{(i_a)}$ for every $a\in \{1,...,m\}$. Upon identifying $L$-labeled edges of $C(\boldsymbol{\tau},\boldsymbol{\eta})$ by $\phi_L$, such trees get joined at their roots. More precisely, if $\phi_L\sim \pi$, then for every block $B=\{j_1,...,j_l\}$ of $\pi$ we obtain the tree $$(\tau^{(j_1)}_{L}\circ\eta^{(j_1)}_{L}\circ \cdots \circ  \tau^{(j_l)}_{L}\circ\eta^{(j_l)}_{L}):=\circ_{i=1}^l(\tau^{(j_i)}_{L}\circ\eta^{(j_i)}_{L}).$$
% For $\phi$ to be acyclic, it must pair edges of such trees internally within each tree. This is explained in figure \ref{fig:tree_partition_rules}, which illustrates how pairings which do not respect this rule give rise to one of two scenarios, each leading to the formation of a cycle. 

% We therefore get, for each block $B=\{j_1,..,j_l\}$ of $\pi$, an acyclic pairing $\phi_B$ of the edges in $\circ_{i=1}^l(\tau_{L}^{(j_i)}\circ\eta_{L}^{j_i})$, of which there are $a_{\circ_{i=1}^l(\tau^{(L)}_{j_i}\circ\eta^{(L)}_{j_i})}:=a_B$ many.

% Lastly, having now paired all $L$--labeled edges belonging to $C(\boldsymbol{\tau},\boldsymbol{\eta})$ (using $\phi_L$) and to the trees of height $L$ decorating this cycle (via the $\phi_{B_1},...,\phi_{B_{|\pi(\phi_L)|}}$), we must pair all remaining edges. 

% Crucially, we observe that these edges are labeled only from $\{1,...,L-1\}$, and form disjoint ``decorated cycles" of their own. More specifically, we obtain such a cycle of length $2\cdot|B^*|\cdot(L-1)$ for each block $|B|^*$ of $\pi^*(\phi_L)$.

% Summarizing what we have so far, an acycling pairing $\phi$ of the edges of $G_k$ must therefore consist of the following:






% \end{proof}



% \textcolor{red}{Anything below this is draft/old text:}


% Further, to avoid the creation of a cycle, edges of such trees can only be paired within the trees themselves. This is explained in figure \ref{fig:}, which illustrates how pairings which do not respect this rule give rise to one of two scenarios, each leading to the formation of a cycle. For each block $B=\{j_1,..,j_l\}$ of $\pi(\phi_L)$, we thus get an acyclic pairing $\phi_B$ of the edges in $\circ_{i=1}^l(\tau^{(L)}_{j_i}\circ\eta^{(L)}_{j_i})$, noting that there are $a_{\circ_{i=1}^l(\tau^{(L)}_{j_i}\circ\eta^{(L)}_{j_i})}:=a_B$ many such pairings.


% \begin{itemize}
%     \item A pairing $\phi_{L}$ of the $L$-labeled edges of $C_k$ for which $\pi(\phi_L)$ is non-crossing.
%     \item For each block $B=\{j_1,..,j_l\}$ of $\pi(\phi_L)$, an acyclic pairing $\phi_B$ of the edges in $\circ_{i=1}^l(\tau^{(L)}_{j_i}\circ\eta^{(L)}_{j_i})$, leading to $=a_B$ many such pairings.
%     \item For each block $B^*=\{m_1,...,m_h\}$ of $\pi^*(\phi_L)$, an acyclic pairing $\phi_{B^*}$ of the edges in 
% \end{itemize}
% This gives a bijection between an acyclic pairings $\phi$ of $G_k$ and triplets $$(\phi_L, \{\phi_B\}_{B\in\pi(\phi_L)}, \tilde{\phi}).$$ and we can therefore write 
% \begin{align*}
% m_{k,L}&=\sum_{{(\boldsymbol{\tau},\boldsymbol{\eta})}} C_{(\boldsymbol{\tau},\boldsymbol{\eta})}a_{G_k(\boldsymbol{\tau},\boldsymbol{\eta})}\\
% &=\sum_{{(\boldsymbol{\tau},\boldsymbol{\eta})}}C_{(\boldsymbol{\tau},\boldsymbol{\eta})}\sum_{\substack{\phi\in \mathcal{P}_{\mathrm{Tree}}(G_k(\boldsymbol{\tau}, \boldsymbol{\eta}))}}1\\
% &=\sum_{(\boldsymbol{\tau},\boldsymbol{\eta})}C_{(\boldsymbol{\tau},\boldsymbol{\eta})}\sum_{\substack{\pi_{L}\in \mathrm{NC_k} \\ \phi_L\sim \pi_L}} \sum_{\tilde{\phi}} 1
% \end{align*}
% \textit{will finish this later, informally want:}
% \begin{align*}
%     \sum_{\pi\in \mathrm{NC}_k} \sum_{\text{joined trees } (\tau',\eta')} C_{\tau',\eta'} \sum_{\substack{\phi_{B},...,\phi_{B_{|\pi|}}\\\text{partition of edges of $(\tau',\eta')$}}} \sum_{\text{rest of edges after $\phi_L$}}\sum_{\tilde{\phi}} C_{\mathrm{the rest}} 
% \end{align*}
% clearly indicating that $\tilde{\phi}$ can be expressed as only depending on $\pi^*$ and noting that we have $\alpha_{joined trees}$ many $\phi_B$'s we can then split this into something of the form
% \[
%     \sum_{\pi\in NC_k} \mu^i m^j
% \]

% \begin{figure}
%     \centering
%     \include{Figures/pifour}
%     \caption{Non-crossing partitions of four vertices and their dual (edge) partitions, up to rotational symmetry.}
%     \label{fig:pifour}
% \end{figure}



% =--------

% From our previous discussion, it is clear that enumerating the graphs in $\mathrm{DC}(\boldsymbol{\ell})$ is equivalent to enumerating all possible choices of trees $\tau_{j}^{(i)},\eta_{j}^{(i)}$ where $j=1,..., \ell_i$ and $i=1,...,k$. We can therefore use express $\mathrm{M}(\boldsymbol{\ell})$ as a sum over trees, writing
% \[
%     \mathrm{M}(\boldsymbol{\ell}) = \sum_{{(\boldsymbol{\tau},\boldsymbol{\eta})=(\tau_{j}^{(i)}, \eta_{j}^{(i)})_{i,j}}} C_{(\boldsymbol{\tau},\boldsymbol{\eta})}a_{G_k(\boldsymbol{\tau},\boldsymbol{\eta})}
% \]
% where $\tau_j^{(i)}\in \bT_{i+1}$ for each $j\in\{0,...,k-1\}, i\in\{0,...,L\}$, so that $(\boldsymbol{\tau},\boldsymbol{\eta})\in (\bT_{L-1}\times\cdots\times \bT_{1})^k$.
% ----



% We are now ready to state the main result of this section.
% \begin{lemma}\label{lemma:FFNNmoments}
%     Let $m_{k,L}$ be as defined above, $\overline{m}_{k,L}:=m_{k,L}/m_{1,L}^k$  and similarly, let $\overline{\mu}_{k,L}=\mu_{k,L}/\mu_{1,L}^k$.
    
%     Then we have
%     \begin{equation}
%                 \overline{m}_{k,L}=1+\sum_{\pi\in \mathrm{NC}_k\setminus \{\{1,...,k\}\}} \sum_{\ell=0}^L \overline{\mu}_{\pi,\ell}\overline{m}_{\pi,\ell-1}.
%     \end{equation}
% \end{lemma}

% We prove the following recurrence formula for $m_{k,L}$, from which lemma \ref{lemma:FFNNmoments} will follow straightfowardly.  
% \begin{lemma}\label{lemma:recurrenceFFNNmoments}
    
% \end{lemma}
% \begin{proof}[Proof of \ref{lemma:FFNNmoments} using \ref{lemma:recurrenceFFNNmoments}] 
% \end{proof}


% To prove lemma \ref{lemma:recurrenceFFNNmoments}, begin by recalling some notation and recalling some from previous sections. Let 
% \[ 
%     \mu_{k, L} := \E{\varphi_{L}'(X)^{2k}}
% \]
% where $X\sim \mathcal{N}(0,K_{L-1}(x,x))$,
% which, using the tree expansion, is equal to 
% %\[
% %    \mu_{k, L}= \lim_{N\to\infty}
% %    \E\bigg(\sum_{\tau, \eta} 
% %    \frac{\varphi_\tau\varphi_\eta}{\sigma(\tau)\sigma(\eta)
% %    }W_{\tau\circ\eta}(x,y)\bigg) 
% %\]
% \[
%     \mu_{k, L}
%     = \sum_{\tau_1, \dots, \tau_{2k} \in \bT_{L}} \left( \prod_i \frac{\dot\varphi_{\tau_i} x^{\tau_i}} {\sigma(\tau_i)}\right)
%     \alpha_{\sqcup_i \tau_i} 
%     = \sum_{\tau_1, \dots, \tau_{2k} \in \bT_{L}} \left( \prod_i \frac{\dot\varphi_{\tau_i} x^{\tau_i}} {\sigma(\tau_i)}\right)
%     a_{\circ_i \tau_i} 
% \]
% where $\circ_i \tau_i$ denotes the tree obtained by joining the trees $\tau_1,\dots,\tau_{2k}$ by their root vertex. and where by $\dot\varphi_{\tau}$ is defined as $\varphi_{\tau}$ under the substitution $\varphi_L \mapsto \varphi'_L$.

% Note here that $\alpha_{\sqcup_i \tau_i} = a_{\circ_i \tau_i}$ since the $\tau_i$ have exactly one root edge and since once two edges have been paired the trees stemming from them must be paired between themselves.

% % \textcolor{red}{justify interchange of $\sum,\mathbb{E},\lim$}
% % \NicoComm{Actually here no need to take E since the convergence is in $L^2$ to the scalars}

% By equation (\ref{jacobianexpansion}), we can write
% \begin{align*}
%     m_{k,L} &= \sum_{\substack{{(\boldsymbol{\tau},\boldsymbol{\eta})}:=(\tau_{i}, \eta_i)_{i=0}^{k-1} \\\in (\bT_{L}^{\rbullet}, \bT_{L}^{\rbullet})^k}}\left(\prod_{i=1}^{k}\frac{\varphi_{\tau_i}\varphi_{\eta_i}}{\sigma(\tau_i)\eta(\tau_i)}\gamma_{\tau_i}\gamma_{\eta_i}\right)\big(\lim_{N\to\infty} \frac{1}{N} \mathbb{E} W_{G_{k}(\boldsymbol{\tau},\boldsymbol{\eta})}\big)\\
%     &:=\sum_{\substack{{(\boldsymbol{\tau},\boldsymbol{\eta})}:=(\tau_{i}, \eta_i)_{i=0}^{k-1} \\\in (\bT_{L}^{\rbullet}, \bT_{L}^{\rbullet})^k}} C_{(\boldsymbol{\tau},\boldsymbol{\eta})}\big(\lim_{N\to\infty} \frac{1}{N} \mathbb{E} W_{G_{k}(\boldsymbol{\tau},\boldsymbol{\eta})}\big)
%  \end{align*}
%  where $G_k(\boldsymbol{\tau},\boldsymbol{\eta})$ is the graph obtained by connecting red n (describe construction of crown of trees)
%  % where $G_k(\tau,\eta)$ is the graph obtained by ``chaining" the trees in the sequence $$(\tau_0, \eta_0, \tau_1, \eta_1,...,\tau_{k-1},\eta_{k-1}),$$ meaning that we connect each tree's (red) output leaf to the root of the next tree in the sequence. \NicoComm{This is not what happens tho, we connect the red nodes in pairs and then connect the roots...}
 
%  Applying theorem \ref{thm:GraphConvergence}, we get 
%  \[
%     \lim_{N\to\infty}\mathbb{E}W_{G_{k}(\boldsymbol{\tau},\boldsymbol{\eta})}=a_{G_k(\boldsymbol{\tau},\boldsymbol{\eta})}, 
%  \]
% reducing the task to counting the number of acyclic pairings of edges of $G_k(\boldsymbol{\tau},\boldsymbol{\eta})$ (as defined in section \ref{sec:genus}). 

% For combinatorial reasons that will soon become apparent, we choose to view a tree in $\bT_{L}$ as a ``trunk" of height $L$ --- which is the path from the root to the output leaf, denoted in red--- to which are attached $L-1$ subtrees of heights $L-1,...,1$ respectively (as depicted in figure \ref{fig:tree_decomposition}). 




% % In other words, we can rewrite the sum in the formula for $m_{k,L}$ as a sum over subtrees, giving
% % \[
% %     m_{k,L}=\sum_{{(\boldsymbol{\tau},\boldsymbol{\eta})=(\tau_{j}^{(i)}, \eta_{j}^{(i)})_{i,j}}} C_{(\boldsymbol{\tau},\boldsymbol{\eta})}a_{G_k(\boldsymbol{\tau},\boldsymbol{\eta})}
% % \]
% % where $\tau_j^{(i)}\in \bT_{i+1}$ for each $j\in\{0,...,k-1\}, i\in\{0,...,L\}$, so that $(\boldsymbol{\tau},\boldsymbol{\eta})\in (\bT_{L-1}\times\cdots\times \bT_{1})^k$.

% % Note that each $G_k(\boldsymbol{\tau},\boldsymbol{\eta})$ is then comprised of a cycle of length $2\cdot k\cdot L$ (formed by the ``trunks" of $\tau_j,\eta_j$), and trees rooted at this cycle's vertices. In particular, a vertex connecting two edges labeled $a$ and $b$ (respectively) in the cycle will be the root of a tree $\tau^{(\mathrm{min}(a,b))}_{j}$ or $\eta^{(\mathrm{min}(a,b))}_{j}$ for some $j\in [k-1]$. This is illustrated in figure \ref{fig:M4crown}.

% % This decomposition of $G_k(\boldsymbol{\tau},\boldsymbol{\eta})$ will simplify the computation of $a_{G_k(\boldsymbol{\tau},\boldsymbol{\eta})}$, which we now undertake. We will denote to the unique cycle in the graph $C_k(\boldsymbol{\tau},\boldsymbol{\eta})$. When it is clear from the context, we will omit the dependence on $(\boldsymbol{\tau},\boldsymbol{\eta})$ for simplicity and use $G_k, C_k$ instead,



% % Furthermore $C_{k,\phi_{L}}$ is a tree if and only if $\pi_{L}$ is non-crossing, in which case we call $\phi_L$ non-crossing as well.
% % \end{lemma}

% % \NicoComm{Should we call $\phi_L$ something like $\phi_{\pi_L}$ instead after this?}

% % % to phrase better: Upon identifying $L$-labeled edges using some $\phi_L$, we're left with decorated cycles of edges labeled $1,...,L_1$, which are joined by trees. After taking care of these trees,  

==> Sections/genus-expansion-section.tex <==
In this section, we develop tools to compute quantities of the form $\E\{\bW_G\}$, where $G$ is a product graph whose edge inputs are matrices with Gaussian entries\footnote{The methods we use extend to non-Gaussian and sparse networks as well, as explored section \ref{sec:non_gaussian}.}. These results are all consequences of Wick's principle, which we now present. For any set $S$ of even size $k$, we define a pairing $\phi$ of $S$ to be a partition of the latter into subsets $S_j=\{\phi_{j,1},\phi_{j,2}\}$ of size two, for $1\leq j\leq k/2$. Then Wick's theorem reduces the task of computing expectations of a product of Gaussian random variables to that of computing pairwise covariances.
\begin{theorem}[Wick's theorem] Let $(Z_i)_{i\geq 1}$ be a complex centered Gaussian vector such that $Z_{-i}=\overline{Z}_i$. Then for any sequence of integers $i_1,...,i_k$, 
\[
\mathbb{E}\Big\{\prod_{j=1}^k Z_{i_j}\Big\} = \sum_{\phi} \prod_{j=1}^{k/2}\mathbb{E}\big\{Z_{i_{\phi_{j,1}}}Z_{i_{\phi_{j,2}}}\big\}.
\]
where the sum is taken over all pairings of $\{1,...,k\}$.
\end{theorem}
Note that the arguments below will, for the most part, resemble those in \cite{dubach2021words}, with some modifications made to accommodate our more general setting. 

\subsection{Wick expansion for product graphs with random inputs} Throughout this section, we will let $\mathcal{W}$ denote the following sequence of random matrices. 
%\JadComm{Note: we can't call them Ginibre because that usually assumes that the matrix is square, and normalizes by the dimension so that one gets the circular law in the limit for the eigenvalues}
\begin{definition}
Let $\mathcal{W}:=(W_i ~|~ i\in \mathbb{Z}\setminus \{0\})$, where for $i>0$, the $W_i\in\mathbb{C}^{N_{r_i}\times N_{c_i}}$ are independent matrices with i.i.d. $\mathcal{N}_{\mathbb{C}}(0,\sigma_i)$ entries. 
For $i<0$, we set $W_{-i}:=\bar{W}_i$ 
and $N_{c_i}=N_{r_{-i}}, N_{r_i}=N_{c_{-i}}$.
\end{definition}
\noindent We will also assume that all of the graphs under consideration satisfy the following assumption, which states that all of the randomness in $G$ must come from $\mathcal{W}$.

\begin{assumption}\label{assumption1} $G$ is a product graph whose inputs are either deterministic, or matrices in $\mathcal{W}$.
\end{assumption}

For any product graph $G$ and edge $e\in E$, we say that $e$ is an ``$\ell$-edge" if its input is fixed to $W_\ell\in \mathcal{W}$.
For simplicity, we label such edges by $\ell$ instead of $W_\ell$ when depicting the graph, as the latter can quickly become cumbersome. 

We will consider pairings of the edges of $G$ whose inputs are matrices in $\mathcal{W}$, denoting the set of such edges by $E_\mathcal{W}$. Such a pairing is said to be \emph{admissible} if it satisfies the following definition.

\begin{definition}[Admissible pairing] 
    Let $G$ be a product graph, and $E_\mathcal{W}=\{e\in E: W_e=W_\ell\text{ for some $\ell(e):=\ell \in \mathbb{Z}\setminus \{0\}$}\}$. Then a pairing $\phi$ of $E_\mathcal{W}$ is said to be \emph{admissible} if any two paired edges $\{e,e'\} \in \phi$ satisfy $\ell(e)=-\ell(e')$. 
    % \[
    %     \exists \ell\in \mathbb{Z}\setminus \{0\} \text{ s.t. }W_e=W_\ell \text{ and } W_{e'}=W_{-\ell}.
    % \]
    We denote the set of all admissible pairings of $E_\mathcal{W}$ by $\mathcal{P}(G)$.
\end{definition}

\begin{figure}[ht]
    \centering
    \vspace{-5pt}
    \scalebox{0.80}{\input{Figures/admissible_partition}}
    \caption{Left: A pairing which is \emph{not} admissible (in red), since a $1$-edge is paired to a $0$-edge and a vertex with input $\mathbf{e}_i$ is paired with one with input $\mathbf{e}_k$. Right: An admissible pairing (in red) and the corresponding $G_{\phi}$ (note that not all edges are necessarily paired).}
    \label{fig:admissible_partition}
\end{figure}

% \begin{figure}
%     \centering
%     \vspace{-5pt}
%     \scalebox{0.80}{\input{Figures/admissible_partition_2}}
%     \caption{Left: A pairing which is \emph{not} admissible (in red), since a $1$-edge is paired to a $0$-edge and a vertex with input $\mathbf{e}_i$ is paired with one with input $\mathbf{e}_k$. Right: An admissible partition (in red) and the corresponding $G_{\phi}$.}
%     \label{fig:admissible_partition_2}
% \end{figure}

% \begin{definition}[Admissible pairing] 
%     Let $G$ be a product graph, and $E_\mathcal{W}=\{e\in E: W_e=W_\ell\text{ for some $\ell\in \mathbb{Z}\setminus \{0\}$}\}$. Then a pairing $\phi$ of $E_\mathcal{W}$ is said to be \emph{admissible} if any two paired edges $e=(u,v), e'=(u',v')$ satisfy
%     \[
%         \exists \ell\in \mathbb{Z}\setminus \{0\} \text{ s.t. }W_e=W_{e'}=W_\ell,
%     \]
%     and $\mathbf{x}_u\odot \mathbf{x}_{u'}$, $\mathbf{x}_v\odot \mathbf{x}_{v'}$ are not equal to a zero vector.
%     We denote the set of all admissible pairings of $E_\mathcal{W}$ by $\mathcal{P}(G)$.
% \end{definition}

% \begin{figure}
%     \centering
%     \vspace{-5pt}
%     \scalebox{0.80}{\input{Figures/admissible_partition}}
%     \caption{Left: A pairing which is \emph{not} admissible (in red), since a $1$-edge is paired to a $0$-edge and a vertex with input $\mathbf{e}_i$ is paired with one with input $\mathbf{e}_k$. Right: An admissible partition (in red) and the corresponding $G_{\phi}$, here $|V_{\boldsymbol{1}}(G_{\phi})| = 2$.}
%     \label{fig:admissible_partition}
% \end{figure}

% For any product graph $G$ and  admissible pairing $\phi\in \mathcal{P}(G)$, let $G_{\phi}$ be the product graph constructed by identifying the edges of $G$ paired by $\phi$ coherently with their orientation (see, e.g., figure \ref{fig:admissible_partition}). The inputs of $G_\phi$ are assigned as follows:
% \begin{itemize}
%     \item When identifying two edges with input $W_\ell$, the resulting edge will also have input $W_\ell$. 
%     \item When identifying two vertices $u,v$ (by pairing edges which have $u$ and $v$ as their respective endpoints), the resulting vertex will have input $\mathbf{x}_u\odot \mathbf{x}_v$. Note that this input is non-zero by definition of an admissible pairing $\phi$.
% \end{itemize} 

For any product graph $G$ and  admissible pairing $\phi\in \mathcal{P}(G)$, let $G_{\phi}$ be the product graph constructed by identifying the edges of $G$ paired by $\phi$ coherently with their orientation (see, e.g., figure \ref{fig:admissible_partition}). 
The inputs of the cells in $G_\phi$ are assigned as follows:
\begin{itemize}
    \item When identifying two edges fixed to  $W_\ell$ and  $W_{-\ell}$, the resulting edge will be fixed to $\E[W_\ell\odot W_{-\ell}] = \sigma_{\ell}^2 \mathbf{I}$.
    \item When identifying two vertices $u,v$ (by pairing edges which have $u$ and $v$ as their respective endpoints), the resulting vertex will have input $\mathbf{x}_u\odot \mathbf{x}_v$. 
\end{itemize} 
Examples of pairings which are and aren't admissible are depicted in figure \ref{fig:admissible_partition}, along with the graph $G_\phi$ that arises in the former case. In the event that it is not connected, we write it as a disjoint union $G_{\phi} = \sqcup_{i=1}^{c(G_{\phi})} (G_i)_{\phi}$ of its connected components $(G_i)_{\phi}$, where $c(G_{\phi})$ denotes the number of connected components of $G_\phi$.


%%%%%%%%%%%%% OLD VERSION %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Lastly, let $V_{\mathbf{1}}(G)$ be the set of vertices of $G$ to which the input is a vector of $1$'s (recalling that such vertices are drawn as $\bullet$, and their inputs are omitted for simplicity). 

% \NicoComm{Find a neat way to restrict this to graphs having only $\boldsymbol{1}$ or $\boldsymbol{e}_i$ as inputs.}
% \JadComm{I agree; this would simplify the proofs of the two lemmas for GP and NTK quite a lot}

% \begin{theorem}\label{thm:wickexpansion}
%  For any (possibly disconnected) product graph $G$,
%     \begin{equation}\label{eq:genusexpansion}
%         \E \left\{W_G \right\}= \sigma_G \sum_{\phi \in \cP(G)} N_{G_{\phi}}.
%     \end{equation}
% where $\phi$ runs over all of $G$'s \emph{admissible} pairings, $N_{G} := \prod_{v \in V_{\boldsymbol{1}}(G)} N_v$
% and  $\sigma_G := \prod_{e \in E(G)} \sigma_{\ell(e)}$.
% \end{theorem}

% The proof is a rewriting of that of Theorem 2.2 in \cite{dubach2021words} in our notation, and itself follows from Wick's theorem. We include it for completeness.
% \begin{proof}
%     Consider the set of indexations
%     \[
%     \mathcal{I}^G := \prod_{v \in V(G)} \{1,...,N_{v}\}
%     \]
%     and recall how for each $\mathbf{i} = (i_v)_{v \in V(G)} \in \mathcal{I}^G$,
%     \[
%     [W_G]_{\mathbf{i}} := \prod_{e = (u,v) \in E(G)} [W_{l(e)}]_{i_u,i_v}
%     \]
%     (see equation \ref{eq:indexation}).  Given $\mathbf{i} \in \mathcal{I}^G$, consider the set of all tuples 
%     \[
%     \mathcal{V}_{\mathbf{i}} := 
%     \{(\{\ell(e),-\ell(e)\},i_u,i_v) : e=(u,v) \in E(G), \ell(e)>0\}
%     \]
%     so that each tuple corresponds to the terms $[W_{\pm\ell(e)}]_{i_ui_v}$ in the product defining $[W_G]_{\mathbf{i}}$.
%     We call an indexation \textit{balanced} if and only if for every $\cv = (\{\ell(e),-\ell(e)\},i_u,i_v) \in \mathcal{V}_{\mathbf{i}}$ the variable
%     $[W_{\ell(e)}]_{i_u,i_v}$ appears in the product defining $[W_G]_{\mathbf{i}}$ as many times as its conjugate $[W^*_{\ell(e)}]_{i_u,i_v}=[W_{-\ell(e)}]_{i_u,i_v}$. 
%     In this case we refer to this number as the \emph{multiplicity} of $\cv$ and denote it by $m_{\cv}$, and write $\mathcal{I}^G_{\mathrm{bal}}$ to denote the set of balanced indexations.

%     If $\mathbf{i}\notin \mathcal{I}^G_{\mathrm{bal}}$, then clearly $\E\{[W_G]_\mathbf{i}\} = 0$. Otherwise, Wick's theorem gives
%     $$
%     \E\{[W_G]_\mathbf{i}\} = \sigma_G \prod_{\cv \in \mathcal{V}_{\mathbf{i}}} m_{\cv}!
%     $$
%     and hence
%     \[
%     \E\{W_G\} = \sigma_G  \sum_{\mathbf{i} \in \mathcal{I}^G_{\mathrm{bal}}}
%     \E\{[W_G]_\mathbf{i}\} = \sigma_G  \sum_{\mathbf{i} \in \mathcal{I}^G_{\mathrm{bal}}}\prod_{\cv \in \mathcal{V}_{\mathbf{i}}} m_{\cv}!
%     \]
%     What's left is to show that this corresponds to the right hand side in equation \ref{eq:genusexpansion}.
%     Given an indexation $\mathbf{i} \in \mathcal{I}^G$ and an \emph{admissible} pairing $\phi \in \mathcal{P}(G)$, we say that $\mathbf{i}$ and $\phi$ are \emph{compatible} if for any paired edges $e=(u,v),e'=(u',v') \in E(G)$ we have $i_u = i_{u'}$ and $i_v = i_{v'}$.It thus follows that there are $\prod_{v \in V(G_{\phi})}N_{v}$ indexations compatible to each admissible $\phi$.
%     Moreover given a balanced $\mathbf{i}$ we can construct a compatible $\phi$ by choosing for every $\cv = (\{\ell(e),-\ell(e)\},i_u,i_v)  \in \mathcal{V}_{\mathbf{i}}$ a pairing between the $m_{\cv}$ copies of $[W_{\ell(e)}]_{i_u,i_v}$ and $[W_{-\ell(e)}]_{i_u,i_v}$ in $[W_G]_{\mathbf{i}}$.

%     This is equivalent to the equality 
%     \[
%     \big|\{(\mathbf{i}, \phi) \in \mathcal{I}^G_{\mathrm{bal}} \times \mathcal{P}(G): \text{$\mathbf{i},\phi$ are compatible} \}\big| 
%     = \sum_{\mathbf{i} \in \mathcal{I}^G_{\mathrm{bal}}}\prod_{\cv \in \mathcal{V}_{\mathbf{i}}} m_{\cv}! = \sum_{\phi \in \mathcal{P}(G)}\prod_{v \in V(G_{\phi}) }N_{v}.
%     \]
% \end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{theorem}[Wick expansion]\label{thm:wickexpansion}
 Let $G$ be a (possibly disconnected) product graph satisfying assumption \ref{assumption1}. Then
    \begin{equation}\label{eq:genusexpansion}
        \E \left\{\bW_G \right\}=  \sum_{\phi \in \cP(G)} \bW_{G_{\phi}}.
    \end{equation}
where $\phi$ runs over all of $G$'s \emph{admissible} pairings.
\end{theorem}

\begin{proof}
    Let $G=(G,\fd, (\mathbf{X}_{c\in C}))$ be a product graph and consider the set of indexations $\mathcal{I}^G := \prod_{v \in V(G)} \{1,...,N_{v}\}$. Recall that for each $e=(u,v)\in E$, $i_e=i_ui_v$. Then for any $\mathbf{i}_V\in \mathcal{I}^G$,
    \[
    \E\Big\{\prod_{c \in C} [\mathbf{X}_c]_{i_c}\Big\} 
        = \prod_{c \in C\setminus E_{\mathcal{W}}} [\mathbf{X}_c]_{i_c}
        \E\Big\{\prod_{e \in E_{\mathcal{W}}} [\mathbf{X}_e]_{i_e}\Big\}.
    \]
    By Wick's theorem, we have
     \begin{align*}
        \E\Big\{\prod_{e \in E_{\mathcal{W}}} [\mathbf{X}_e]_{i_e}\Big\} =& 
         \sum_{\phi} \prod_{\{e,e'\} \in \phi } \E\Big\{ [\mathbf{X}_e]_{i_e} [\mathbf{X}_{e'}]_{i_{e'}}\Big\}
    \end{align*}
    where the sum is over all pairings $\phi$ of $E_{\mathcal{W}}$. Note that if $\phi\notin \cP(G)$ then 
    $$\prod_{\{e,e'\} \in \phi } \E\Big\{ [\mathbf{X}_e]_{i_e} [\mathbf{X}_{e'}]_{i_{e'}}\Big\} = 0$$ 
    and we can therefore write
    \begin{align}\label{eq:W_Glemma}
        \E\{\mathbf{W}_G\} =& 
        \sum_{\mathbf{i}_V} 
        \left(
        \prod_{c \in C\setminus E_{\mathcal{W}}} [\mathbf{X}_c]_{i_c}
        \right)
        \sum_{\phi \in \cP(G)} \prod_{\{e,e'\} \in \phi } 
        \E\Big\{ [\mathbf{X}_e]_{i_e} [\mathbf{X}_{e'}]_{i_{e'}}\Big\}
        % \nonumber \\ =&
        % \sum_{\phi \in \cP(G)} \sum_{\mathbf{i}_V} 
        % \left(
        % \prod_{c \in C\setminus E_{\mathcal{W}}} [\mathbf{X}_c]_{i_c}
        % \right)
        % \prod_{\{e,e'\} \in \phi } 
        % \E\Big\{ [\mathbf{X}_e]_{i_e} [\mathbf{X}_{e'}]_{i_{e'}}\Big\}
        \nonumber \\ =&
        \sum_{\phi \in \cP(G)} \sum_{\mathbf{i}_V} 
        \left(
        \prod_{c \in C\setminus E_{\mathcal{W}}} [\mathbf{X}_c]_{i_c}
        \right)
        \prod_{\{e,e'\} \in \phi } \sigma_{\ell(e)}^{2} \delta_{i_e,i_{e'}},
    \end{align}
    % Define the set $$V_{\mathcal{R}} := \{v \in V(G) ~|~  \exists e \in E_{\mathcal{W}}, \exists u \in V(G) \text{ s.t. } e = (v,u) \text{ or } e = (u,v)\}$$ then we can conclude by noticing that for any $\phi \in \cP(G)$, by definition
    where $\delta_{i,j} := \mathbf{1}(i=j)$ is the Kronecker delta function.
    
    %  Now let $V_{\mathcal{R}}$ be the set of vertices which are adjacent to edges of $E_{\mathcal{W}}$, and note how an admissible pairing $\phi$ induces a partition $V_{\mathcal{R}}(\phi)$ of $V_{\mathcal{R}}$, into sets of vertices which were identified as a result of their adjacent edges being identified by $\phi$.
    % Note that a similar definition for the edges would result in $E_{\mathcal{W}}(\phi) = \phi$.
    % There we have the following canonical bijections
    % \[
    % V(G_\phi) \simeq V_{\mathcal{R}}^{c} \sqcup V_{\mathcal{R}}(\phi), \quad
    % E(G_\phi) \simeq E_{\mathcal{W}}^{c} \sqcup E_{\mathcal{W}}(\phi) = E_{\mathcal{W}}^{c} \sqcup \phi.
    % \]
    % Given $u \in V_{\mathcal{R}}$ let us write $\boldsymbol{\pi}(u)$ for the $\pi \in V_{\mathcal{R}}(\phi)$ such that $u \in \pi$, if instead  $u \in V_{\mathcal{R}}^c$ we set $\boldsymbol{\pi}(u):=u$;
    % in other words, $\boldsymbol{\pi}$
    % \footnote{$\boldsymbol{\pi}$ depends on $\phi$, we decided to omit this dependence in the notation given that this $\phi$ will always be fixed.} 
    % associates to any vertex $u \in V(G)$ the corresponding one in $V(G_{\phi})$ obtained after the identifications induced by $\phi$.
    % We extend $\mathbf{\pi}$ to $E$ by setting $\boldsymbol{\pi}(u,v) = (\boldsymbol{\pi}(u),\boldsymbol{\pi}(v))$.
    For any vertices $u,v\in V$, we say that they are $\phi$-equivalent and write $u\sim_\phi v$ if they are identified after identifying edges according to $\phi$. Similarly, we write $e\sim_\phi e'$ if $\{e,e'\}\in \phi$. If we let $V_\mathcal{R}$ be the set of vertices adjacent to edges in $E_\mathcal{W}$, we then have canonical bijections
    \[
        V(G_\phi)\simeq V_\mathcal{R}^c \sqcup (V_\mathcal{R}/\sim_\phi),\quad E(G_\phi)\simeq E^c_\mathcal{R} \sqcup (E_\mathcal{W}/\sim_\phi)\,
    \]
    Note that each element in $\varepsilon\in E_\mathcal{W}/\sim_\phi$ corresponds to a block $\varphi(\varepsilon)\in \phi$, while each element of $\nu\in V_\mathcal{R}/\sim_\phi$ corresponds to a subset $\varphi(\nu)\subset V$ (these are the pre-images under the quotient maps).  
     Then for any $\phi\in \mathcal{P}(G)$ we can write the product of $G_{\phi}$ in terms of indexations of $G$ as
    \begin{align*}
        \bW_{G_{\phi}} =& 
        \sum_{\mathbf{i}\in \mathcal{I}^{G_{\phi}}} 
        \prod_{c \in E_{\mathcal{W}}^c \cup V_{\mathcal{R}}^c} [\mathbf{X}_c]_{i_c}
        \left( 
        \prod_{\varepsilon\in (E_\mathcal{W}/\sim_\phi)} \sigma_{\ell(\varepsilon)}^{2} 
        %\underbrace{[\mathbf{I}]_{i_{\varphi(\varepsilon)}}}_{1}
        \right) 
        \left(
        \prod_{\nu \in (V_\mathcal{R}/\sim_\phi)} \prod_{u \in \varphi(\nu)}[\mathbf{X}_u]_{i_\nu}
        \right)
        \\
        =& 
        \sum_{\mathbf{i}\in \mathcal{I}^{G}} 
        \prod_{c \in E_{\mathcal{W}}^c \cup V_{\mathcal{R}}^c} [\mathbf{X}_c]_{i_c}
        \left( 
        \prod_{\{e,e'\} \in \varphi(\epsilon) } \sigma_{\ell(e)}^{2}
        \delta_{i_e,i_{e'}}
        \right) 
        \left(
        \prod_{\nu \in (V_\mathcal{R}/\sim_\phi)} 
        \delta_{\mathbf{i}|_\nu}
        \prod_{u \in \varphi(\nu)}[\mathbf{X}_u]_{i_u} 
        \right)
    \end{align*}
    Here $\delta_{\mathbf{i}|_\nu} := \mathbf{1}\left(\forall u,u' \in \varphi(\nu). ~i_u=i_{u'}\right)$ and $\sigma_{\ell(\varepsilon)} = \sigma_{\ell(e)}$ for any choice of $e \in \varphi(\varepsilon)$, since they all yields the same $\sigma_{\ell(e)}$.
     Given that, by definition, $\exists \nu \in (V_\mathcal{R}/\sim_\phi)$ such that $u,v \in \varphi(\nu)$ if and only if $\exists \{e,e'\}\in\phi$ such that $u$ and $u'$ are corresponding bordering vertices, it follows that the term $\delta_{\mathbf{i}|_\nu}$ is superfluous in the sense that 
     \[
     \prod_{\{e,e'\} \in \varphi(\epsilon)} \delta_{i_e,i_{e'}} =
     \prod_{\nu \in (V_\mathcal{R}/\sim_\phi)} \delta_{\mathbf{i}|_\nu}.
     \]
     Using this, the claim then follows from the equality
    \[
    \prod_{c \in C\setminus E_{\mathcal{W}}} [\mathbf{X}_c]_{i_c} = 
    \left( \prod_{c \in E_{\mathcal{W}}^c \cup V_{\mathcal{R}}^c} [\mathbf{X}_c]_{i_c} \right)
    \left(
    \prod_{\nu \in (V_\mathcal{R}/\sim_\phi)} 
    \prod_{u \in \varphi(\nu)}[\mathbf{X}_u]_{i_u} 
    \right).
    \]
\end{proof}
% By a straightforward application of the Euler characteristic formula, this result generalizes the \emph{Genus Expansion} of \cite{dubach2021words} to our more general setting. 
% Indeed, the latter considers products of traces $\mathrm{Tr}(M_{w_i})$ where each $M_{w_i}$ is a word of $N\times N$ complex Ginibre matrices. As explained in section \ref{subsect:unlabeled_case}, such products can be expressed as the values of polygonal product graphs, with edges labeled by the letters of $w_i$ and vertices with inputs $\boldsymbol{1}_N$.

We now use this result to derive a centered version of it (proposition \ref{prop:mixedmoments_}), which we will need to derive limit theorems for $\mathbf{W}_{G}$.
To that end, we need to single out the following types of admissible pairings which largely dictate its first and second-order behaviour.

\begin{definition}
    Let $G = \sqcup_{i=1}^{c(G)} G_{i}$ be a product graph, given as a disjoint union of its connected components, and fix an admissible pairing $\phi \in \cP(G)$ of its edges.
    \begin{enumerate}
        \item $\phi$ is said to be \emph{fully-atomic} if and only if for every $1\leq i\leq c(G)$, the edges of $G_i$ are paired within themselves $(G_i)_{\phi|_{G_i}}$ is a tree for each $i$, where $\phi|_{G_i}$ denotes the pairing induced by $\phi$ on the edges of $G_i$.
        %, and $(G_i)_{\phi|_{G_i}}$ denotes the graph obtained from $G_i$ after identifying edges paired by $\phi|_{G_i}$).
        \item $\phi$ is \emph{bi-atomic} if and only if \emph{no} $G_i$ is paired within itself, the $G_i$ are paired in pairs and each of the paired components $(G_i \sqcup G_j)_{\phi|_{G_i \sqcup G_j}}$ is a tree.
        \item $\phi$ is \emph{atom-free} if and only if \emph{no} $G_i$ is paired within itself to form a tree.
    \end{enumerate}
\end{definition}
We denote the set of (admissible) fully-atomic, bi-atomic and atom-free pairings of $G$ by $\mathcal{P}_{\mathrm{A}}(G)$, 
$\mathcal{P}_{\mathrm{bi}}(G)$, and $\mathcal{P}_{\mathrm{AF}}(G)$  respectively. 
With these definitions, we can now state and prove the following centered version of theorem \ref{thm:wickexpansion}.
\begin{proposition}\label{prop:mixedmoments_}
Let $G=\sqcup_{i=1}^{c(G)}G_i$ be a product graph satisfying assumption \ref{assumption1}, with disjoint connected components $G_i$.Then
\begin{equation}\label{eqn:lemma:fix_vertices_new}
     \E\bigg\{
     \prod_{i=1}^{c(G)} \Big( 
     \bW_{G_i} - 
    \sum_{\psi \in \mathcal{P}_{\mathrm{A}}(G_{i})}
      \bW_{(G_i)_\psi}
     \Big)
     \bigg\} = 
     \sum_{\phi \in \mathcal{P}_{\mathrm{AF}}(G)} \bW_{G_\phi}
\end{equation}
\end{proposition}

\begin{proof}
Let $[c(G)]:=\{1,...,c(G)\}$, and for any $T \subseteq [c(G)]$ define $G_{T} := \sqcup_{i \in T} G_i$. Then by expanding the expectation in (\ref{eqn:lemma:fix_vertices_new}), we get
    \begin{align*}
        \mathbb{E}\bigg\{
        \prod_i &\Big(W_{G_i} -
        \sum_{\psi \in \mathcal{P}_{\mathrm{A}}(G_{i})}
         \bW_{(G_i)_\psi}\Big)\bigg\}
         \\
        &=
        \sum_{T \subseteq [c(G)]} (-1)^{|T^c|} \E\left\{ \prod_{i \in T} \bW_{G_i} \right\} %\sigma_{G_{T^c}}
        \left( \prod_{i \notin T} 
       \sum_{\psi \in \mathcal{P}_{\mathrm{A}}(G_{i})}
        \bW_{(G_i)_{\psi}}
        \right)
    \end{align*}
 Using theorem \ref{thm:wickexpansion}, we have
\[
\E\bigg\{\prod_{i \in T} \bW_{G_i} \bigg\} = \sum_{\phi \in \mathcal{P}(G_T)}
     \bW_{(G_T)_{\phi}}
\]
and in turn
\begin{align*}
    &=  
\sum_{T \subseteq [c(G)]} \sum_{\phi \in \cP(G_T)}
(-1)^{|T^c|}
\bW_{(G_T)_{\phi}}
\prod_{i \notin T} 
       \sum_{\psi \in \mathcal{P}_{\mathrm{A}}(G_{i})}
     \bW_{(G_i)_{\psi}}  
     \\
     &= 
        \sum_{T \subseteq [c(G)]} 
        (-1)^{|T^c|}
        \sum_{\phi \in \cP(G_T) \times (\times_{i \in T^c} \mathcal{P}_{\mathrm{A}}(G_i))}
        \bW_{G_{\phi}}
\end{align*}
\NicoComm{Should we put $\times$ instead of $\sqcup$?}
and the conclusion follows from the inclusion-exclusion principle since 
\[
\mathcal{P}_{\mathrm{AF}}(G) = \bigcap_{i=1}^{c(G)} (\mathcal{P}(G_{[c(G)]\setminus \{i\}}) \times \mathcal{P}_{\mathrm{A}}(G_i))^c = \mathcal{P}(G) \setminus \bigcup_{i=1}^{c(G)} \big(\mathcal{P}(G_{[c(G)]\setminus \{i\}}) \times \mathcal{P}_{\mathrm{A}}(G_i)\big)
\]
and 
\[
\bigcap_{i \in T^c} \big( \mathcal{P}(G_{[c(G)]\setminus \{i\}}) \times \mathcal{P}_{\mathrm{A}}(G_i)\big) = \cP(G_T) \times_{i \in T^c} \mathcal{P}_{\mathrm{A}}(G_i).
\]
\end{proof}

More generally the same proof shows:
\begin{proposition}
    Let $G=\sqcup_{i=1}^{c(G)}G_i$ be a product graph satisfying assumption \ref{assumption1}, with disjoint connected components $G_i$. 
    Given any sequence $\cP_i \subseteq \cP(G_i)$ and setting $\cP_{\star} := \bigcap_i [\cP(G_{[c(G)]\setminus\{i\}}) \sqcup \cP_i]^c$ one has
\begin{equation}
     \E\bigg\{
     \prod_{i=1}^{c(G)} \Big( 
     \bW_{G_i} - 
    \sum_{\psi \in \cP_i}
      \bW_{(G_i)_\psi}
     \Big)
     \bigg\} = 
     \sum_{\phi \in \cP_{\star}} \bW_{G_\phi}
\end{equation}
\end{proposition}



\subsection{Genus Expansion}
\label{sec:genus_actual}

We now study a particular setting in which it will be possible to explicitly express all the values $\mathbf{W}_{G_{\phi}}$.

% \begin{assumption}\label{assumption:genus_graph}
%     For the sequence $\mathcal{W}$ we assume all $N_{c_i} = N_{r_i} = N$ for some integer $N>0$.
%     We will consider product graphs $G$ such that for all $v\in V$ one has $\fd(v)=N$, $\mathbf{X}_v = \mathbf{1}_N$ and $E_{\mathcal{W}}(G) = E$.
% \end{assumption}

\begin{assumption}\label{assumption:genus_graph}
      $\mathcal{W}$ is such that all $N_{c_i} = N_{r_i} = N$ for some integer $N>0$, and $G$ is such that $\fd(v)=N$, $\mathbf{X}_v = \mathbf{1}_N$ for all $v\in V$ and $\mathbf{X}_e = \mathbf{I}$ for all $e \in E\setminus E_{\mathcal{W}}(G)$.
\end{assumption}

Under assumption \ref{assumption:genus_graph}, the definition of $\bW_{G_\phi}$ then directly yields
\begin{equation}\label{eq:allones}
    \bW_{G_\phi} = \sigma_G N^{V(G_\phi)}, \quad \sigma_G = \prod_{e\in E_{\mathcal{W}}}\sigma_{\ell(e)}.  
\end{equation}
given that all the edges of $G_\phi$ are labeled by $\mathbf{I}_{N \times N}$.
The order of $\bW_{G_\phi}$ is thus determined by the number of vertices in $G_\phi$. 

Instead of counting the latter directly, it is often simpler to associate a surface to $G_\phi$ and use its Euler characteristic to express $|V(G_\phi)|$ in terms of this surface's genus, number of edges and connected components. This forms the basis of the \textit{genus expansion} technique, which has been used extensively to compute random matrix integrals.

To use it, we will need some basic notions from topological graph theory (see \cite{GrossTucker} for a more in-depth introduction). Any connected graph $G=(V,E)$ can be viewed as a topological space, by viewing vertices as distinct points and edges as subspaces homeomorphic to $[0,1]$ joining their ends, such that edges only meet at their endpoints. 
An \textit{embedding} $\rho$ of $G$ on some orientable surface $S$ is then defined as a homeomorphism from $G$ (viewed as a space) to $S$. 
The connected components of $S\setminus\rho(G)$
are referred to as the \textit{faces} of the embedding, and we denote the total number of faces by $f(G:S)$. 
The genus of $S$ is denoted by $g(S)$.
\begin{proposition}[Euler's formula] Let $\rho$ be an embedding of a connected $G=(V,E)$ on an orientable surface $S$. Then we have
\[
    |V|-|E|+f(G:S)=2-2g(S).
\]
\end{proposition}

\noindent Further, it is well known that all orientable surfaces of genus $g$ are equivalent up to homeomorphism (as a representative of their equivalence class, one can for instance take the surface obtained by adding $g$ ``handles" to a $2$-sphere, see \cite{Brahana}). For any $g\geq 0$, it thus makes sense to talk about \textit{the} surface of genus $g$, which we henceforth denote by $S_g$. 

Lastly, we can define embeddings of disconnected graphs by considering each connected component separately. Letting $c(G)$ denote the number of components and $G=\sqcup_{i=1}^{c(G)} G_i$, an embedding of $G$ is given by embedding each $G_i$ on an oriented surface $S_i$. We can also extend the definitions of $f$ and $g$ by writing  $S=\sqcup_{i=1}^{c(G)}S_i$,\[
    g(S):=\sum_{i=1}^{c(G)}g(S_i),\quad \text{ and }f(G:S)=\sum_{i=1}^{c(G)}f(G_i:S_i),
\]
and we note that Euler's formula still applies.

\bigskip

Going back the setting of assumption \ref{assumption:genus_graph}, let $G$ be such a product graph and $\phi\in \mathcal{P}(G)$ be an admissible pairing of its edges. Recalling that $G_\phi$ is the graph obtained from $G$ after identifying edges paired by $\phi$, we let
\[
    S_\phi := \min_g \{S_g:\ \text{there exists an embedding } \rho:G_\phi\to S_g\}.
\]
if $G$ is connected. Otherwise, let $(S_i)_{\phi}$ be the surface obtained this way from each connected component $G_i$ of $G$, and define $S_\phi = \sqcup_{i=1}^{c(G)} (S_i)_{\phi}$.

\begin{remark}
    Note how given such a $G$ and \emph{any} $\phi \in \cP(G)$ the graph $G_{\phi}$ always the same number of edges, this number is
    \begin{equation}
        \check{e}(G) := |E(G_{\phi})| = |E_\mathcal{W}(G)|/2+|E\setminus E_{\mathcal{W}}(G)|
    \end{equation}
    since the random edges are identified in pairs, and the rest are left untouched.
\end{remark}

Theorem \ref{thm:wickexpansion} then yields the following.
\begin{corollary}[Genus Expansion]
\label{thm:wickexpansion_ones}
Let $G$ be a product graph satisfying assumptions \ref{assumption1} and \ref{assumption:genus_graph}.
Then for any $\phi\in \mathcal{P}(G)$,
\begin{equation}
    \bW_{G_\phi} = \sigma_{G}N^{2(c(G_\phi)-g(S_\phi))-f(G_\phi;S_\phi)+\check{e}(G)},
\end{equation}
and it follows that
\begin{equation}
    \E \left\{ \bW_G \right\} = \sigma_G N^{\check{e}(G)} \sum_{\phi \in \cP(G)} N^{2(c(G_\phi)-g(S_\phi))-f(G_\phi;S_{\phi})}.
\end{equation}
\end{corollary}

\begin{proof}
This follows directly from equation (\ref{eq:allones}) and Euler's formula, noting that the latter yields
\begin{equation}
|V(G_{\phi})| =  2(c(G_{\phi})-g(S_{\phi})) + |E(G_\phi)| - f(G_{\phi}: S_{\phi}).
\end{equation}
\end{proof}

This result can be seen as a generalization of the expansion in \cite{Dubach2021} to our setting. Indeed, the latter considers products of traces $\mathrm{Tr}(M_{w_i})$ where each $M_{w_i}$ is a word of $N\times N$ complex Ginibre matrices. As explained in the following example, such products can be expressed as the values of polygonal product graphs.
\begin{example}
    Under assumption \ref{assumption:genus_graph}, let $w$ be a word of matrices in $\mathcal{W}$. If, for instance, $w=W_1W_4^TW_2^TW_5W_3^T$, then taking  $G$ to be the product graph in figure \ref{fig:polygon-word} below gives $\mathbf{W}_G=\mathrm{Tr}(w)$.
    \begin{figure}[ht]
        \centering
        \input{Figures/polygon_word}
        \caption{A product graph whose value is the trace of a word of Ginibre random matrices.}
        \label{fig:polygon-word}
    \end{figure}
    
    Theorem 2.2 in \cite{Dubach2021} can then be recovered from corollary \ref{thm:wickexpansion_ones} by considering disjoint unions of such graphs. 
\end{example}


In this specific setting we can have a more specific centered result to study mixed moments:
\begin{lemma}\label{lemma:mixedmoments_genus}
Let $G$ satisfy assumptions \ref{assumption1} and \ref{assumption:genus_graph}. Then for every $\phi\in \cP_{AF}(G)$, we have $$2(c(G_\phi)-g(S_\phi))-f(G_\phi;S_{\phi})\leq  \frac{c(G)}{2}. $$
Further, equality holds if and only if $\phi$ is bi-atomic, giving
\begin{equation*}
    \E\left\{\prod_{i=1}^{c(G)} 
    \left(W_{G_i}-\sigma_{G_i} N^{\check{e}(G_i)+1} |\mathcal{P}_\mathrm{A}(G_i)| \right)\right\} = \sigma_G N^{ \check{e}(G) + \frac{c(G)}{2} } \left(|\mathcal{P}_\mathrm{bi}(G)|+\mathcal{O}\left(\frac{1}{N}\right) \right).
\end{equation*}
\end{lemma}

\begin{proof}
    Assume that $
    c(G_{\phi}) \leq {c(G)}/{2}
    $.
    Then it suffices to prove that for each connected component $G_i$ of $G$ and its corresponding surface $S_i$, 
    \[
    2(1-g((S_i)_\phi))-f\big((S_i)_\phi;(S_i)_{\phi}\big) \leq 1
    \]
    and that the equality holds if and only if $(G_i)_\phi$ is a tree.

    
    Since $f\big((G_i)_\phi;(S_i)_{\phi}\big) \geq 1$ and $g\big((S_i)_\phi\big) \geq 0$, we have 
    \[
    2(1-g\big((S_i)_\phi)\big)-f\big((G_i)_\phi;(S_i)_\phi\big) 
    \leq 
    2(1-0)-1 = 1
    \]
    with equality if and only if $f\big((G_i)_\phi;S^{(i)}_{\phi}\big) = 1$ and $g\big((S_i)_\phi\big) = 0$ (which is equivalent to $(G_i)_\phi$ being a tree).
    Now if $c(G_{\phi}) > {c(G)}/{2}$ instead, then there must be at least     
    \[
    2\bigg(c(G_{\phi}) - \frac{c(G)}{2}\bigg)
    \]
    components of $G_\phi$ of the form $(G_j)\big|_{\phi}$ for some $1\leq j\leq c(G)$. Letting $k$ be the number of components obtained this way, then we must have that $k \geq 2(c(G_{\phi}) - {c(G)}/{2})$: assuming otherwise, the inequality 
    \[
    c(G) \geq k + 2(c(G_{\phi}) - k) = 2\bigg(c(G_{\phi}) - \frac{k}{2}\bigg)
    \]
    quickly gives a contradiction. Since $\phi$ is atom-free, 
    \[
    f((G_i)_\phi;(S_i)_\phi) = 1 \implies g((S_i)_\phi) > 0
    \]
    for these components, and it follows that
    \[
    2(1-g\big((S_i)_\phi\big)-f\big((G_i)_\phi;(S_i)_\phi\big) \leq 0.
    \]
    As for the remaining components (of which there are strictly less than $c(G)/2$) this quantity is $\leq 1$ as proved above, and the lemma follows.
\end{proof}

\begin{corollary}
Let $G$ be a product graph satisfying assumptions \ref{assumption1} and \ref{assumption:genus_graph}, and $\lambda_G := \frac{1}{\sigma_{G} N^{\check{e}(G)+1}}$ 
    \begin{equation}
    \E\left\{ 
    \left(\lambda_G W_{G}- |\mathcal{P}_\mathrm{A}(G_i)| \right)^2 \right\} = \frac{1}{N} \left(|\mathcal{P}_\mathrm{bi}(G)|+\mathcal{O}\left(\frac{1}{N}\right) \right)
\end{equation}
\end{corollary}


Combining the previous two results yields the following limit theorem for the joint distribution of product graphs. 
\begin{theorem}\label{thm:joint_gaussian_limit}
    Let $(G_i)_{i\geq 1}$ be a sequence of connected product graphs satisfying assumptions \ref{assumption1} and \ref{assumption:genus_graph}. Then for any $m\geq 1$,
    \[
        \big((\sigma_{G_i}N^{\check{e}(G_i) + \frac{1}{2}}\big)^{-1}\bW_{G_i} - a_{G_i} \sqrt{N})_{i=1}^m \overset{d}{\longrightarrow} \mathbf{Z} = \big(Z_1,...,Z_m\big)^{\top}
    \]
    where the limit is a centered complex Gaussian vector with covariance function  $C := \E[\mathbf{Z}\mathbf{Z}^{\top}]$
    having entries $[C]_{i,j} = \alpha_{G_i \sqcup G_j}$ and pseudo covariance $\Gamma := \E[\mathbf{Z}\mathbf{Z}^{H}]$ with entries $[\Gamma]_{i,j} = \alpha_{G_i \sqcup G^*_j}$.
\end{theorem}

\begin{proof}
    We use the moment method. Setting 
    \[
    \tilde Z_i := (\sigma_{G_i}N^{\check{e}(G_i) + \frac{1}{2}})^{-1}\bW_{G_i} - a_{G_i} \sqrt{N}
    \]we want to compute the expectations
    \[
    \E\left\{ \prod_{i=1}^m (\tilde Z_i)^{k_i} (\tilde Z_i^*)^{l_i}\right\}
    \]
    for non-negative integers $k_i, l_i$.
    We are in the setting of Lemma \ref{lemma:mixedmoments_genus} and the leading term of the expectation is the number of bi-atomic pairings of the induced graph.
    Given a possible pairing of its connected components, for each of its pairs $(\tilde G, \tilde G')$ this contributes a factor $\alpha_{\tilde G \sqcup \tilde G'}$ to the total sum. 
    But this is exactly the result of computing 
    \[
    \E\left\{ \prod_{i=1}^m (Z_i)^{k_i} ( Z_i^*)^{l_i}\right\}
    \]
    by applying Wick's theorem. Hence we conclude.
\end{proof}

\begin{comment}
\subsection{The labeled leaves case}
\NicoComm{Move this to the GP Lim place}
Here we consider the more general case in which the vertices are either labeled by $\boldsymbol{1}_{N_v}$ or by a basis element $e_k$, but the latter can occur only if the degree of the vertex is $1$.
In other words we consider those graphs where the labeled vertices only appear as "leaves" in a general sense. 

\begin{proposition}\label{prop:mixedmoments_2}
%Let $v_{\boldsymbol{1}, \mathrm{bi}}(G)$ be the number of unlabeled vertices \NicoComm{This should be the number that \emph{would be} in...}in any \emph{bi-atomic} pairing of $G$, similarly $v_{\boldsymbol{1}, \mathrm{A}}(G)$
%will be the number of such vertices in any \emph{fully-atomic} pairing of the graph.
Given a graph $G$ let $e(G):=|E(G)|$ and $v(G):=|V(G)|$ be, respectively, the cardinality of the set of edges and vertices.
Defining 
\begin{equation}
    v_{\boldsymbol{1}, \mathrm{A}}(G_i) = \frac{e(G_i)-v(G_i) + v_{\boldsymbol{1}}(G_i)}{2}+1, \quad v_{\boldsymbol{1}, \mathrm{bi}}(G) = \frac{e(G)- v(G) + v_{\boldsymbol{1}}(G)}{2} + \frac{c(G)}{2},
\end{equation}
then for all compatible graphs where labeled vertices all have degree $1$
it holds
\begin{equation}\label{eqn:lemma:fix_vertices}
     \E\left\{\prod_{i=1}^{c(G)} \left[W_{G_i}-\sigma_{G_i} N^{v_{\boldsymbol{1}, \mathrm{A}}(G_i)}a_{G_i}\right]\right\} = \sigma_G N^{v_{\boldsymbol{1}, \mathrm{bi}}(G)} \left(\alpha_{G}+O\left(\frac{1}{N}\right) \right).
\end{equation}
\end{proposition}

\begin{theorem}\label{thm:joint_gaussian_limit_2}
    Let $(G_i)_{i\geq 1}$ be a sequence of graphs as above. Then for any $m\geq 1$,
    \[
        ((\sigma_{G_i}N^{v_{\boldsymbol{1}, \mathrm{A}}(G_i) - \frac{1}{2}})^{-1}W_{G_i} - a_{G_i} \sqrt{N})_{i=1}^m \overset{d}{\longrightarrow} \mathbf{Z} = (Z_1,...,Z_m)^{\top}
    \]
    where the limit is a centered complex Gaussian vector with covariance function  $C := \E[\mathbf{Z}\mathbf{Z}^{\top}]$
    having entries $[C]_{i,j} = \alpha_{G_i \sqcup G_j}$ and pseudo covariance $\Gamma := \E[\mathbf{Z}\mathbf{Z}^{H}]$ with entries $[\Gamma]_{i,j} = \alpha_{G_i \sqcup G^*_j}$.
\end{theorem}

\end{comment}

% \subsection{The Real Case}
% \JadComm{I think it's correct, this admissibility criterion encapsulates Dubach-Peled's ``direct and indirect" pairings in the real case}
% \NicoComm{I will need to understand more fully their view, I always am confused}
% \JadComm{The more I read this, the more I think that the whole thing would flow much better if we do everything complex up to section 5, then have a section 5(b) that expands everything to real, non-gaussian and sparse. Alternatively, hoping that the real case isn't much more complicated than the complex one, do everything for the real case from the get go, then talk about non-gaussian/sparse/complex extensions in section 5(b). The back and forth right now is confusing and unnecessary}

% The {real case} corresponds to the following setting:

% % I have a little Haiku for you
% % this stays: :)
% % over these pages
% % friends lurk in a sea words
% % good mathematics




% \begin{assumption}
% Let $\mathcal{W}:=(W_i ~|~ i\in \mathbb{N})$, where for $i>0$, the $W_i\in\mathbb{R}^{N_{r_i}\times N_{c_i}}$ are independent matrices with real i.i.d. $\mathcal{N}(0,\sigma_i)$ entries. 
% \end{assumption}

% Under this assumption the results hold \emph{verbatim} if one considers the following notion of \emph{admissibility}:
% \begin{definition}[Admissible pairing of edges with real-valued inputs] 
%     Let $G$ be a product graph, and $E_\mathcal{W}=\{e\in E: W_e=W_\ell\text{ for some $\ell(e):=\ell \in \mathbb{N}$}\}$. Then a pairing $\phi$ of $E_\mathcal{W}$ is said to be \emph{admissible} if any two paired edges $\{e,e'\} \in \phi$ satisfy $\ell(e)=\ell(e')$. 
% \end{definition}

% Only theorem \ref{thm:joint_gaussian_limit} has to be reworded, forgetting about the pseudo-covariance, as:
% \begin{theorem}\label{thm:joint_real_gaussian_limit}
%     Under assumption \ref{assumption:genus_graph},
%     let $(G_i)_{i\geq 1}$ be a sequence of connected product graphs. Then for any $m\geq 1$,
%     \[
%         \big((\sigma_{G_i}N^{\check{e}(G_i) + \frac{1}{2}}\big)^{-1}\bW_{G_i} - a_{G_i} \sqrt{N})_{i=1}^m \overset{d}{\longrightarrow} \mathbf{Z} = \big(Z_1,...,Z_m\big)^{\top}
%     \]
%     where the limit is a centered complex Gaussian vector with covariance function  $C := \E[\mathbf{Z}\mathbf{Z}^{\top}]$
%     having entries $[C]_{i,j} = \alpha_{G_i \sqcup G_j}$.
% \end{theorem}


==> Sections/graph-dictionary.tex <==
Our objective, which we achieve in section \ref{sec:genus}, is to use the genus expansion technique to study matrix/vector products arising in the study of neural networks. The latter turn out to be best described by directed graphs, and this section develops a dictionary between graphs and analytic operations which will lie at the foundation of all of our results. 

\subsection{Product graphs}

% In what follows, all of the vectors and matrices are assumed to be complex-valued, (we treat the real-valued case using similar arguments in section \ref{sec:extensions}).
% \begin{assumption}
%      In what follows, $\mathcal{W} := ((W_i, N_{r_i}, N_{c_i}) : i \in \mathbb{Z}\setminus\{0\})$, where for $i>0$, $W_i \in \bC^{N_{r_i} \times N_{c_i}}$ are independent \emph{complex} Ginibre matrices and $(W_{-i}, N_{c_{-i}}, N_{r_{-i}}) := (W_{i}^*, N_{c_{i}}, N_{r_{i}})$.
% \end{assumption}

Consider a directed graph $G=(V,E)$. We associate a vector $\mathbf{X}_v\in \mathbb{C}^{\fd(v)}$ to each vertex $v\in V$ and a matrix $\mathbf{X}_e\in \mathbb{C}^{\fd(u)\times \fd(v)}$ to each edge $e=(u,v)\in E$, calling $\mathbf{X}_e$ and $\mathbf{X}_v$ the \textit{inputs} of their respective edge/vertex. Here, $\fd(v)$ is a positive integer which call the \textit{dimension} of the vertex $v$, and we extend $\fd$ to edges by using the shorthand $\fd(e)=(\fd(u),\fd(v))$ for $e=(u,v)\in E$ (in which case $\mathbb{C}^{\fd(e)}:=\mathbb{C}^{\fd(u)\times \fd(v)}$).

As we are often going to talk about vertices and edges simultaneously, it will be useful to have a single term to refer to both types of objects. For this purpose we will use the term \emph{cells}, as is customary in algebraic topology, noting that this fits in with possible generalizations of the tools developed here (e.g. by considering simplicial complexes instead of graphs, see Section \textcolor{orange}{???}). Every cell in $V\cup E$ will thus have a  dimension assigned to it by $\fd$, noting that this map is entirely determined by the values that it takes on vertices.

As we will soon make precise, $G$ can be seen as describing a type of product of its inputs. This motivates the naming in the following definition, which summarizes what we have introduced so far. 
\begin{definition}[Product graph]\label{def:product-graph}
    A \emph{product graph} is a sequence $(G,\fd, \mathfrak{C})$, where 
    \begin{itemize}
        \item $G=(V,E)$ is a directed graph with vertex set $V$ and edge set $E\subseteq V\times V$.
        \item  $\fd$ assigns a dimension to each vertex, thus to each cell of $G$.
        \item $\mathfrak{C}=(\mathbf{X}_c)_{c\in C}$ is a sequence of vectors/matrices associated to the cells of $G$.
    \end{itemize}
    Furthermore, $\mathfrak{C}$ is \textit{compatible} with $\fd$, meaning that any cell $c\in C :=  V\cup E$ is associated to an input $\mathbf{X}_c \in \mathbb{C}^{\fd(c)}$.
\end{definition}

% We will say that the matrices and vectors are \emph{fixed} to the corresponding cells, pictorially this will be reflected by labeling each cell by the corresponding matrix/vector as in figures \ref{fig:path-graph} and \ref{fig:basic-tree}.

When $\fd$, $\mathfrak{C}$ are clear or implied from the context, we will omit them and simply use $G$ to denote the entire product graph. The product defined by $G$ is then given by the following definition, and its outcome is referred to as the \textit{value} of $G$.

\begin{definition}
    Let $(G,\fd,\mathfrak{C})=G$ be a product graph. Then the \emph{value} of $G$ is the product
\begin{equation}\label{eq:product}
        \bW_G:=\sum_{\mathbf{i}_{V}} \prod_{c \in C}~
        [\mathbf{X}_c]_{i_c} \in \bC
\end{equation}
where the sum is taken over all \textit{indexations} $\mathbf{i}_{V} = (i_v)_{v\in V} \in \prod_{v\in V} \{1,...,N_v\}$ and
where for $c = (u,v) \in E$ we define $i_c := i_ui_v$.
% \begin{equation}\label{eq:product}
%         \bW_G:=\sum_{\mathbf{i}_{V}} ~[W_G]_{\mathbf{i}_{V}}\prod_{v\in V}[\mathbf{x}_v]_{i_v} \in \bC
% \end{equation}
%     and 
% \begin{equation}\label{eq:indexation}
%         [W_G]_{\mathbf{i}_{V}} = \prod_{e=(u,v)\in E}[W_e]_{i_u,i_v}.
% \end{equation}
\end{definition}

Note that the compatibility condition in Definition \ref{def:product-graph} ensures that this product is well-defined. Furthermore, if $G$ is disconnected and has connected components $\{G_i\}_i$, then $\bW_G=\prod_{i} \bW_{G_i}$. In the event that some of its inputs are random, $\bW_G$ then becomes a random variable (this will be done in later sections to study neural networks).

We now illustrate this definition with the following examples. 
\begin{example}
If $G$ is the product graph in figure \ref{fig:path-graph}, then $\bW_G=\mathbf{x}_a^{\top}W_3W_2W_1\mathbf{x}_d$ since 
\[
\mathbf{x}_a^{\top}W_3W_2W_1\mathbf{x}_d = \sum_{\alpha,\beta,\gamma,\delta} [W_3]_{\alpha,\beta} [W_2]_{\beta,\gamma} [W_3]_{\gamma,\delta} [\mathbf{x}_a]_{\alpha} [\mathbf{x}_d]_{\delta} 
\]
\begin{figure}[ht]
    \centering
    \input{Figures/pathgraph.tex}
    \caption{A product graph giving rise to a word of matrices multiplied by vectors on either side. $\mathbf{1}_{N}$ is the $N\times 1$ vector of $1$s.}
    \label{fig:path-graph}
\end{figure}
\end{example}
\begin{example}
    Hadamard (entry-wise) products of matrices arise when $G$ is a tree. For instance, taking $G$ to be the product graph in figure \ref{fig:basic-tree}
    gives
    \[  
    \bW_G=\mathbf{x}_a^{\top} W_2\big(\mathbf{x}_{b} \odot (W_1\mathbf{x}_d)\astrosun(W_1\mathbf{x}_c)\big)
    \]
    where $A\astrosun B$ denotes the entry-wise product of $A$ and $B$.
    % \footnote{The labels $a,b,c,d$ given to the vertices are there only to keep track of the different vertices. If this is implied/clear from the context, we will omit them from the notation.}.
    In fact the product is
    \[
    \bW_G := \sum_{\alpha,\beta,\gamma,\delta} [W_2]_{\alpha,\beta}[W_1]_{\beta,\gamma}[W_1]_{\beta,\delta} 
    [\mathbf{x}_{a}]_{\alpha}[\mathbf{x}_{b}]_{\beta}
    [\mathbf{x}_{c}]_{\gamma}[\mathbf{x}_{d}]_{\delta}
    \]
    \begin{figure}[ht]
        \centering
        \input{Figures/basic-tree.tex}
        \caption{A product graph with tree structure
        .}\label{fig:basic-tree}
    \end{figure}
\end{example}
Note that while the examples above can be described in terms of ordinary matrix/vector multiplication and entry-wise products, this isn't necessarily the case for more general graphs. 

% \textcolor{red}{So I think this should stay as-is until here, and this is where we properly introduce the choice of in/out/free vertices and the multilinear maps. We then proceed to (shamelessly) call that map $\bW_G$, but justify that by saying that if the in/out/free vertices are the empty set, then this map coincides with our previous definition of $W_G$ in that it's just the constant map equal to the value of the product graph.}
\bigskip
\subsection{Operator graphs and their associated linear map} \JadComm{Important: this section is not correct as-is; we're ignoring the fact that the input/output cells need to have an order so that the tensor products make sense. Thankfully the rest remains correct, as all of our analysis just happens to be order-inariant (e.g. only one input/output, or using the law of total differential when we have more inputs, in which case the sum commutes.}So far, we have associated a vector/matrix to each cell in our graphs. 
By \emph{freeing} some of these cells, meaning that we consider their inputs as variables, we can use graphs to define more general linear maps between tensor spaces.

Consider for example the product graph $(G,\fd,\mathfrak{C})=G$ in figure \ref{fig:basic-tree}, noting how the product defining $\bW_G$ is {linear} in $\bx_a$. If we consider $\bx_a$ to be a variable, this yields a well-defined linear map $\bC^{\fd(a)} \to \bC$ or, via {Riesz representation}, a vector in $\bC^{\fd(a)}$.
In this particular case, the linear map in question would be $\bx \mapsto \bx^{\top} W_2\big(\mathbf{x}_{b} \odot (W_1\mathbf{x}_d)\astrosun(W_1\mathbf{x}_c)\big)$, and its vector representation is $W_2\big(\mathbf{x}_{b} \odot (W_1\mathbf{x}_d)\astrosun(W_1\mathbf{x}_c)\big)$. 

\bigskip

More generally, let $G$ be a directed graph with dimensions assigned by $\fd$, and let $\mathcal{F}$ be the set of {free} cells of $G$ (meaning the vertices and edges which are considered as variables) assuming that the remaining cells are \textit{fixed} to some inputs $(\mathbf{X}_c)_{c\in C\setminus \mathcal{F}}$. Then for any choice of inputs $(\mathbf{X}_c)_{c\in \mathcal{F}}$, the product defining $\mathbf{W}_{(G,\fd,(\mathbf{X}_c)_{c\in C})}=\mathbf{W}_G$ is $|\mathcal{F}|-$linear in these inputs, or equivalently, linear in $\otimes_{c\in \mathcal{F}}\mathbf{X}_c$ by the universal property of tensor products.

Furthermore, given any a partition of $\mathcal{F}$ into two subsets $\mathcal{F}_\mathrm{in}$ and $\mathcal{F}_{\mathrm{out}}$, we can consider the map
\begin{equation}\label{eq:associatedmap1}
    \otimes_{c\in \mathcal{F}_{\mathrm{in}}}\mathbf{X}_c \mapsto \big(\otimes_{c\in \mathcal{F}_{\mathrm{out}}}\mathbf{X}_c \mapsto \mathbf{W}_G\big).
\end{equation}
This is equivalent to considering the map
\begin{equation}\label{eq:associatedmap2}
        \otimes_{c\in \mathcal{F}_{\mathrm{in}}}\mathbf{X}_c \mapsto \mathbf{Y},\quad \langle \mathbf{Y}, \otimes_{c\in \mathcal{F}_\mathrm{out}}  \mathbf{X}_{\mathrm{c}}\rangle= \mathbf{W}_G\, \text{ for any } (\mathbf{X}_c)_{c\in \mathcal{F}_{\mathrm{out}}}    
\end{equation}
where $\mathbf{Y} \in \bigotimes_{c\in \mathcal{F}_{\mathrm{out}}} \mathbb{C}^{{\fd}(c)}$ is the Riesz representation of $\big(\otimes_{c\in \mathcal{F}_{\mathrm{out}}}\mathbf{X}_c \mapsto \mathbf{W}_G\big)$.

This map is then linear, and its input and output dimensions depend on the partition of $\mathcal{F}$ that is being taken. We refer to it as the \textit{operator associated to} $G$, as defined below.

\begin{definition}[Operator associated to a graph]\label{def:operator-graph}
    An \emph{operator graph} is a sequence 
    $(G,\fd,\mathcal{F}_{\mathrm{in}},\mathcal{F}_{\mathrm{out}},(\mathbf{X}_c)_{c\in C\setminus\mathcal{F}}),$ where  
    \begin{itemize}
        \item $G=(V,E)$ is a directed graph,
        \item $\fd$ is its dimension function,
        \item  $\mathcal{F}=\mathcal{F}_{\mathrm{in}}\sqcup\mathcal{F}_{\mathrm{out}}$ is the set of free cells in $G$, partitioned into subsets of \textit{in} and \textit{out} cells,
        \item $(\mathbf{X}_c)_{c\in C\setminus\mathcal{F}}$ is a sequence of inputs associated to the {fixed} cells of $G$, which are compatible with $\fd$ (as defined in \ref{def:product-graph}).
    \end{itemize}
    Then the operator associated to this $(G,\fd,\mathcal{F}_{\mathrm{in}}, \mathcal{F}_{\mathrm{out}},(\mathbf{X}_c)_{c\in C\setminus\mathcal{F}})=G$ is defined as
    \begin{equation*}
        \mathbf{W}_G: \bigotimes_{c\in \mathcal{F}_{\mathrm{in}}} \mathbb{C}^{\fd(c)} \to \bigotimes_{c\in \mathcal{F}_{\mathrm{out}}} \mathbb{C}^{\fd(c)}, \quad\mathbf{W}_G[\otimes_{c\in \mathcal{F}_{\mathrm{in}}} \mathbf{X}_c]=\mathbf{Y}
    \end{equation*}
    where $\mathbf{Y}$ is the unique vector satisfying
        $\sprod{\mathbf{Y}}{\otimes_{c\in \mathcal{F}_{\mathrm{out}}}\mathbf{X}_c} = 
        \bW_{(G,\fd,(\mathbf{X}_c)_{c\in C})}$.
\end{definition}

Note that we used the same notation as for the value of a product graph. This is to reflect the fact that operator graphs essentially reduce to the latter when $\mathcal{F}=\emptyset$, recalling that the empty tensor product is defined as the base field $\mathbb{C}$. Indeed, the operator associated to $(G,\fd, \emptyset,\emptyset,(\mathbf{X}_c)_{c\in C})$ is
\[
    \quad z\mapsto \mathbf{W}_{(G,\fd,(\mathbf{X}_c)_{c\in C})}z, \quad z\in \mathbb{C}.
\]
Just as we did for product graphs, we will abuse notation and just use $G$ to denote an  operator graph when $\mathcal{F}_{\mathrm{in}},\mathcal{F}_{\mathrm{out}}, (\mathbf{X}_c)_{c\in C\setminus \mathcal{F}}$ and $\fd$ are clear from the context. We thus use $\mathbf{W}_G$ to denote both an operator (when $G$ is an operator graph) and a scalar (when $G$ is a product graph).
\bigskip

Some examples to illustrate these definitions might be in order, and are given below. When depicting a graph, a free vertex is drawn as a circle (e.g. $\circ$) and is blue if it is in $\mathcal{F}_{\mathrm{out}}$, while a vertex fixed to $\mathbf{x}$ is drawn as a black dot labeled by said vector (e.g. $\bullet_{\mathbf{x}}$). 
Similarly, we draw free edges with dotted directed lines (e.g. $\dashrightarrow$) and in blue if they are in $\mathcal{F}_{\mathrm{out}}$, while fixed edges are drawn as solid lines labeled by their input matrix (e.g. $\xrightarrow[]{W}$).

For simplicity, we will omit labels from vertices (resp. edges) whose input is $\mathbf{1}$ (resp. $\mathbf{I}$) when drawing them.

\begin{example}
Let $G$ be the graph in figure \ref{fig:basic-tree-free} (left). To turn this into an operator graph, let $a,b,c,d$ refer to its vertices from bottom to top/ left to right and let $\fd:\{a,b,c,d\}\to\mathbb{N}$ be any fixed dimension map. Then if we consider $\cF_{\mathrm{in}} = \{d,(a,b)\}$ and $\cF_{\mathrm{out}} = \{a\}$ and fix the remaining cells as (\emph{cf.} figure \ref{fig:basic-tree-free})
\[
b \mapsto \mathbf{x}_b, ~
c \mapsto \mathbf{1}, ~ 
(b,d) \mapsto \mathbf{I}, ~
(b,c) \mapsto W_1
\]
we obtain the linear map
$\mathbf{x}_d \otimes W_{(a,b)} \mapsto 
W_{(a,b)}
\big(\mathbf{x}_{b} \odot (W_1\mathbf{1})\astrosun(\mathbf{I} ~\mathbf{x}_d)\big) \in \bC^{\fd(a)}$.
%If we take the leaves (vertices of out-degree $0$) of this tree to be free vertices (the result is depicted in figure \ref{fig:basic-tre--free} below), then $W_{(G, (\mathbf{x}_b),(W_1))}=W_G$ is the 2-linear map
% \[
% (\mathbf{x}_c,\mathbf{x}_d, W_{(a,b)}) \mapsto 
% \mathbf{x}_a^{\top}W_2\big(\mathbf{x}_{b} \odot (W_1\mathbf{x}_d)\astrosun(W_1\mathbf{x}_c)\big)
% \]
    \begin{figure}[ht]
    \centering
    
    \input{Figures/basic-tree-free}
    \caption{Example of an operator graph (right) obtained from a graph (left) by a choice of $\mathcal{F}_{\mathrm{in}}$, $\mathcal{F}_{\mathrm{out}}$, $\fd$ and $(\mathbf{X}_c)_{c\in C\setminus \mathcal{F}}$. Note how on the right, we omit labels from vertices and edges whose inputs are $\mathbf{1}$ or $\mathbf{I}$ respectively.}%, obtained from the graph in figure \ref{fig:basic-tree} by taking the leaves as free vertices. }
    \label{fig:basic-tree-free}. 
\end{figure}

% \end{example}

%  A particularly relevant case for later sections is that of $G$ having exactly two free vertices $a,b\in V$ such that $\cF_{\mathrm{in}} = \{a\}, ~ \cF_{\mathrm{out}}=\{ b\}$. In that case, the operator $\bW_G$ is a linear map $\bC^{\fd(a)} \to \bC^{\fd(b)}$ (\emph{i.e.} it is a matrix of size $\fd(b) \times d(a)$). When evaluated at some vector $\mathbf{x}_a$, the output 
%  \begin{example}
%      If $G$ is the operator graph in figure \ref{fig:Riesz_Graphs} (left), then its associated map $\mathbf{W}_G$ is from $\mathbb{C}^{\fd(a)}\to\mathbb{C}^{\fd(b)}$. Evaluating this map at some vector $\mathbf{x}_a$ thus yields a vector in $\mathbb{C}^{\fd(b)}$; graphically, this vector is given by the graph in
%  \end{example}

%  Note how the matrix $\bW_G^{\top}$ is just the operator $\bW_{G^{\top}}$ corresponding to the operator graph $G^{\top}$ constructed from $G$ by simply exchanging the \emph{in/out} roles of vertices $a,b$.

 

% \begin{example}


%  \begin{figure}
 
%         \centering
%         \scalebox{0.90}{\input{Figures/Riesz_Graphs}} 
%         \caption{}
%         \label{fig:Riesz_Graphs}
% \end{figure}

% \NicoComm{I removed the letters from the boxes...}

\end{example}




% \NicoComm{Can this be removed?}
% \begin{example}
%     Taking $G$ to be the graph in figure \ref{fig:first-example}, all of whose vertices are free, we find that
%    $W_{(G,\ell,\emptyset)}=W_G$ is the map defined by
%     \[(\mathbf{x}_a,\mathbf{x}_b,\mathbf{x}_c,\mathbf{x}_d)\mapsto\sum_{(i_a,i_b,i_c,i_d)} [W_G]_{(i_a,i_b,i_c,i_d)}[\mathbf{x}_a]_{i_a} [\mathbf{x}_b]_{i_b} [\mathbf{x}_c]_{i_c} [\mathbf{x}_d]_{i_d} 
%    \]
% where
%     \[
%     [ W_G ]_{(i_a, i_b, i_c, i_{d} )} = 
%     [W_3]_{i_a,i_b }
%     [W_3]_{ i_a, i_{d}}
%     [W_2]_{i_{b}, i_c}
%     [W_2]_{i_d, i_c}
%     \]
%     where $1\leq i_a\leq d(a)$ and similarly for $i_b,i_c$, and $i_d$. This quantity is described by the product graph obtained by associating an input to each free vertex in $G$ (see figure \ref{fig:first-example}, right).
% \begin{figure}[!h]
%         \centering
%         \input{Figures/first-example}
%         \caption{A directed graph with four free vertices,  to which we can associate a $4$-linear map (left). Given input $(\mathbf{x}_a,\mathbf{x}_b,\mathbf{x}_c,\mathbf{x}_d)$, this map evaluates to the value of the product graph on the right.}
%         \label{fig:first-example}
% \end{figure}
% \end{example}


\subsection{Operations on graphs.}\label{dictionary} Having outlined the correspondence between graphs and operators, we can now go further and show how various analytic operations can be expressed as binary operations on graphs.


\begin{definition}[Fixing a free cell] Let $(G,\mathfrak{d}, \mathcal{F}_{\mathrm{in}}\sqcup\mathcal{F}_{\mathrm{out}}, (\mathbf{X}_c)_{c\in C})$ be an operator graph, $\mathbf{W}_G$ its associated map and $c_0\in \mathcal{F}_{\mathrm{in}}\sqcup\mathcal{F}_{\mathrm{out}}$ be a free cell of $G$. Then if $G|_{c_0:\mathbf{Y}}$ is the graph obtained by fixing $c_0$'s input to some $\mathbf{Y}$, we have
\[
    \mathbf{W}_{G|_{c_0:\mathbf{Y}}}[\otimes_{c\in\mathcal{F}_\mathrm{in}}\mathbf{X}_c]=
    \begin{cases}
        \mathbf{W}_G[\mathbf{Y}\otimes_{c\in\mathcal{F}_\mathrm{in}}\mathbf{X}_c] & \text{if } c\in \mathcal{F}_{\mathrm{in}}\\
        \text{\textcolor{red}{to fill}} & \text{if } c\in \mathcal{F}_{\mathrm{out}}.\\
    \end{cases}
\]
\end{definition}

For example, let $G$ be the operator graph on the left in figure \ref{fig:fixing} below. Then $$\mathbf{x} \mapsto (\mathbf{y} \mapsto \mathbf{x}^{T}[ W_{2}[( W_{1}\mathbf{1}) \odot ( W_{1}\mathbf{y})]).$$ If we fix the free out-vertex of $G$ to $\mathbf{Y}_0$ (c.f. figure \ref{fig:fixing}, middle), we get the map
    \[
        \mathbf{x} \mapsto \mathbf{x}^{T} W_{2}[ W_{1}\mathbf{1} \odot W_{1}\mathbf{Y}_{0}]
    \]
    while fixing the in-vertex (c.f. figure \ref{fig:fixing}, right)
    \[
        \mathbf{y} \mapsto \mathbf{Y}_{0}^{T}[ W_{2}[( W_{1}\mathbf{1}) \odot ( W_{1}\mathbf{y})]].
    \]
    \vspace{-10pt}
\begin{figure}[ht]
    \centering
    \include{Figures/fixing}
    \vspace{-10pt}
    \caption{Fixing a free out-vertex (middle) and in-vertex (right) of a graph.}
    \label{fig:fixing}
\end{figure} 



For any operator graph $(G,\mathfrak{d},\mathcal{F}_{\mathrm{in}},\mathcal{F}_{\mathrm{out}}, (\mathbf{X}_c)_{c\in C})$, recall that $\mathbf{W}_G$ is linear by definition and thus corresponds to a vector in $\prod_{c\in \mathcal{F}_{\mathrm{out}}}\mathbb{C}^{\mathfrak{d}(c)}\times \prod_{c\in \mathcal{F}_{\mathrm{in}}}\mathbb{C}^{\mathfrak{d}(c)}$. It will therefore make sense to talk about coordinates of $\mathbf{W}_G$, and to take Hadamard products between $\mathbf{W}_{G_1}$ and $\mathbf{W}_{G_2}$, for instance. 

% In particular, if $\mathcal{F}_{\mathrm{out}}=\{v\}$ and $\mathcal{F}_{\mathrm{in}}=\{u\}$ for some vertices $v,u$ of $G$, then $\mathbf{W}_G$ is simply a $\mathfrak{d}(u)\times \mathfrak{d}(v)$ matrix.

\begin{definition}[Identifying free vertices] 
Let $G_1=(G_1,\fd_1, \emptyset, \{v_1\}, (\mathbf{X}_c)_{c\in C_1})$ and $G_2=(G_2,\fd_2, \emptyset, \{v_2\}, (\mathbf{X}_c)_{c\in C_2})$ be operator graphs with a unique free vertex $v_1\in V(G_1)$ and $v_2\in V(G_2)$ respectively. Assume that they are out-vertices, and that $\fd_1(v_1) = \fd_2(v_2)$. 
Then $G_1 \wedge G_2$ is defined as the graph obtained by identifying $v_1$ and $v_2$, meaning
\[
    G_1 \wedge G_2 := (G_1\cup G_2)/\{v_1=v_2\}.
\]
Note that since $G_1$ and $G_2$ have only one free cell, $\mathbf{W}_{G_1}, \mathbf{W}_{G_2}$ and $\mathbf{W}_{G_1\wedge G_2}$ all correspond to unique vectors in $\mathbb{C}^{\fd_1(v_1)}$. We then have that $\bW_{G_1 \wedge G_2} = \bW_{G_1} \odot \bW_{G_2} \in \bC^{\fd(v_1)}$. 
\end{definition}

\begin{figure}[ht]
    \centering
    \include{Figures/identifying}
    \vspace{-20pt}
    \caption{Identifying two graphs by their unique free vertex corresponds to taking a Hadamard product of their associated operators. Here, the fixed vertices of $G_1$ and $G_2$ are all assumed to have input $\mathbf{1}$.}
    \label{fig:identifying}
\end{figure}
This operation can straightforwardly be extended for generic operator graphs which have more than one free cell, in which case one should specify the cells being identified. This will not be needed for our purposes, and we thus opt for the definition above in an effort to keep our notation simple. 

Note that the graph operation $\wedge$ is associative and symmetric much like its analytic counterpart $\odot$, meaning that there is no confusion in writing $G_1 \wedge \cdots \wedge G_n = \bigwedge_{i \in [n]} G_i$.    

\begin{definition}[Switching in and out vertices]\label{def:swap_vertices}
Let $G=(G,\mathfrak{d},\{u\}, \{v\}, (\mathbf{X}_c)_{c\in C})$ be an operator graph with exactly two free vertices $u$ and $v$, one of which is an out-vertex. Note that in this case, $\mathbf{W}_G$ is a ${\mathfrak{d}(u)}\times {\mathfrak{d}(v)}$ matrix. Then if
\[
    G^T:=(G,\mathfrak{d},\{v\}, \{u\}, (\mathbf{X}_c)_{c\in C}),
\]
 it is easy to see that $\mathbf{W}_G^T=\mathbf{W}_{G^T}$.
\begin{figure}[ht]
        \centering
        \input{Figures/transposition}
        \caption{Transpose of an operator graph.}\label{fig:transposition}
\end{figure}
\end{definition}
Once again, one can make this definition more general by considering any choice of $\mathcal{F}_{\mathrm{in}}$ and $\mathcal{F}_{\mathrm{out}}$, and swapping these two sets in their entirety. We chose to highlight a much simpler situation in the previous example, as it will be of particular use to us in later sections.

\begin{definition}[Composition]
Let $G_1=(G_1,\fd_1, \mathcal{F}^{(1)}_{\mathrm{in}},\mathcal{F}^{(1)}_{\mathrm{out}}, (\mathbf{X}_c)_{c\in C_1\setminus \mathcal{F}_1})$ and $G_2=(G_2,\fd_2, \mathcal{F}^{(2)}_{\mathrm{in}},\mathcal{F}^{(2)}_{\mathrm{out}}, (\mathbf{X}_c)_{c\in C_2\setminus \mathcal{F}_2})$ be operator graphs, $c_1\in \mathcal{F}^{(1)}_{\mathrm{in}},c_2\in \mathcal{F}^{(2)}_{\mathrm{out}}$ be a pair of edges or of vertices satisfying $\fd_1(c_1)=\fd_2(c_2)$. Then the \emph{composition} $G_1\circ G_2$ of these graphs is the graph obtained by identifying $c_1$ and $c_2$ and fixing the resulting cell's input to $\mathbf{1}$ or $\mathbf{I}$ accordingly. Note that if any vertices $v_1, v_2$ are identified as a result (e.g., when $c_1,c_2$ are edges), the resulting vertex is given input $\mathbf{x}_1\odot \mathbf{x}_2$ where $\mathbf{x}_1,\mathbf{x}_2$ are the respective inputs of $v_1$ and $v_2$. Then we have
\[  
    \mathbf{W}_{G_1\circ G_2} = \mathbf{W}_{G_1}\circ \mathbf{W}_{G_2}
\]
where on the right hand side, $\circ$ denotes composition of maps.
\end{definition}
\JadComm{Need to once again show dependence on the cells in the notation, but then say we omit it in the simple case. How to make this non-repetitive?}
For instance, consider two operator graphs $$G_1=(G_1, \mathfrak{d}_1, \{a\}, \{b\}, (\mathbf{X}_c)_{c\in C_1\setminus \{a,b\}}), G_2=(G_2, \mathfrak{d}_2, \{b'\}, \{c\}, (\mathbf{X}_c)_{c\in C_2\setminus \{b',c\}}),$$ and assume that $\mathfrak{d}_1(b)=\fd_2(b')=N$ for some $N>0$. Then the product $\bW_{G_1} \bW_{G_2}$ is a matrix with coordinates 
$$[\bW_{G_1} \bW_{G_2}]_{\alpha,\gamma} = \sum_{\beta = 1}^{N} [\bW_{G_1}]_{\alpha,\beta} [\bW_{G_2}]_{\beta,\gamma} = \sum_{\beta = 1}^{N} [\bW_{G_1}]_{\alpha,\beta} [\bW_{G_2}]_{\beta,\gamma} [\boldsymbol{1}]_{\beta}$$
and the right hand side is exactly $\mathbf{W}_{G_1\circ G_2}$.

\begin{figure}[ht]
        \centering
        \input{Figures/composition_edges}
        \caption{Composition of two vertices (left) and edges (right).}
        \label{fig:composition_edges}
\end{figure}

A concrete example of the case in which the two cells are edges $e,e'$  will be given in section \ref{sec:NTK} when computing the Neural Tangent Kernel.

% \[
% \iota_x: V  \to V\otimes W, \quad v \mapsto v\otimes x
% \]
% \[
% \sprod{\iota_x(v)}{v'\otimes w'} = \sprod{v \otimes x}{v'\otimes w'} 
% = \sprod{v}{v'}\sprod{x}{w'} = \sprod{v}{\sprod{x}{w'}  v'}
% \]

% \[
% \iota_x^* :  V\otimes W \to V, \quad v \otimes w \mapsto \sprod{x}{w} v 
% \]

\begin{definition}[Trace]
Let $G=(G,\mathfrak{d},\{c_1\}, \{c_2\}, (\mathbf{X}_c)_{c\in C})$ be an operator graph with exactly two free cells $c_1$ and $c_3$, one of which is an out-vertex, and such that $\fd(c_1)=\fd(c_2)$.
Then the \emph{trace} $\mathrm{Tr}(G)$ of $G$ is the graph obtained by identifying $c_1$ with $c_2$ and fixing the resulting cell to $\mathbf{1}$ or $\mathbf{I}$ accordingly. Again, if any vertices $v_1, v_2$ are identified as a result (e.g., when $c_1,c_2$ are edges), the resulting vertex is given input $\mathbf{x}_1\odot \mathbf{x}_2$ where $\mathbf{x}_1,\mathbf{x}_2$ are the respective inputs of $v_1$ and $v_2$.
Then we have 
\[
\mathrm{Tr}(\bW_G) = \bW_{\mathrm{Tr}(G)}.
\]
\end{definition}

For instance consider $G=(G,\mathfrak{d},\{a\}, \{b\}, (\mathbf{X}_c)_{c\in C})$ in figure \ref{fig:traces}, assuming $\fd(a)=\fd(b)=N$. Then
\[
\mathrm{Tr}(\bW_G) = \sum_{\alpha=1}^N [\bW_G]_{\alpha,\alpha} = \sum_{\alpha=1}^N [\bW_G]_{\alpha,\alpha} [\boldsymbol{1}]_{\alpha}
=\bW_{\mathrm{Tr}(G)}
\]
Note how the trace can be seen as composition which is ``internal to a graph".
\begin{figure}[ht]
        \centering
        \input{Figures/traces}
        \caption{Trace of a graph.}
        \label{fig:traces}
\end{figure}


\begin{definition}[Differential]\label{def:graphdiff}
    Let $G=(G,\fd, \mathcal{F}_{\mathrm{in}},\mathcal{F}_{\mathrm{out}}, (\mathbf{X}_c)_{c\in C \setminus \mathcal{F}})$ be an operator graph. 
    Assume fixed an ordering of $\mathcal{F}_{\mathrm{in}}$ corresponding to the sequence $\mathfrak{c} := (c_1, \dots, c_{|\mathcal{F}_{\mathrm{in}}|})$. 
    Fix also a sequence $\mathbf{X}_{\mathfrak{c}} := (\mathbf{X}_{c_1}, \dots,  \mathbf{X}_{|\mathcal{F}_{\mathrm{in}}|})$ of possible corresponding inputs. Then the \emph{differential} of $G$ in the sequence $\mathbf{X}_{\mathfrak{c}}$ is the linear combination of operator graphs 
    \[
    (dG)_{\mathbf{X}_{\mathfrak{c}}} := 
    \sum_{i=1}^{|\mathcal{F}_{\mathrm{in}}|}
    (d_iG)_{\mathbf{X}_{\mathfrak{c}}}
    \]\JadComm{Should we define a graph algebra so that the differential is itself a graph? }
    where $(d_iG)_{\mathbf{X}_{\mathfrak{c}}} := (G,\fd, \{c_i\},\mathcal{F}_{\mathrm{out}}, (\mathbf{X}_c)_{c\in C \setminus \mathcal{F}_{G}} \sqcup \mathbf{X}_{\mathfrak{c}\setminus\{c_i\}})$ has only $c_i$ as in-cell since all other cells of $\cF_{\mathrm{in}}(G)$ have been fixed to the corresponding elements from $\mathbf{X}_{\mathfrak{c}}$.

    Note that we can consider the linear operator $\bW_G$ as a multilinear map 
    \[
        \bW_G^{\mathfrak{c}} : \prod_{i = 1}^{|\mathcal{F}_{\mathrm{in}}|} \bC^{\fd(c_i)} \to \bigotimes_{c \in \cF_{\mathrm{out}}} \bC^{\fd(c)}
    \]
    then under this identification, using the law of total differential, we have
    \[
    (d\bW_G^{\mathfrak{c}})_{\mathbf{X}_{\mathfrak{c}}} 
    = \sum_{i=1}^{|\mathcal{F}_{\mathrm{in}}|}
    (d_i \bW_{G}^{\mathfrak{c}})_{\mathbf{X}_{\mathfrak{c}}} = \sum_{i=1}^{|\mathcal{F}_{\mathrm{in}}|}
    \bW_{(d_iG)_{\mathbf{X}_{\mathfrak{c}}}}= 
    \bW_{(dG)_{\mathbf{X}_{\mathfrak{c}}}} 
    \]
\end{definition}



% Our graphs define multi-linear maps, thus they are equal to their own differentials with respect to any of their inputs, corresponding to the free cells. 
% The law of total differential then tells us that the differential with respect to \emph{all} the inputs of a $\bW_G$ is represented just by the sum of as many copies of the original graph as there are free cells, where in each copy the corresponding cell is to be fixed to a differential direction (\emph{cf.} figure \ref{fig:derivative}). 

\begin{figure}[ht]
        \centering
        \input{Figures/derivative}
        \caption{Example of derivation of a graph with the product graph resulting from the evaluation of the derivative.}
        \label{fig:derivative}
\end{figure}

\begin{figure}[ht]
        \centering
        \input{Figures/derivative_2}
        \caption{The differential at point $(\mathbf{x}_{a},\mathbf{x}_{b}, W)$ of operator $\bW_G$ in figure \ref{fig:derivative}.}
        \label{fig:derivative_2}
\end{figure}

% If an ordering of the $m$ free cells and a corresponding sequence $\mathfrak{c} := (\mathfrak{c}_1, \dots, \mathfrak{c}_m)$ of inputs are specified, then we can write without ambiguity that $(\mathrm{d}\bW_{G})_{\mathfrak{c}} = \sum_{i=1}^m \bW_{(\mathrm{d}_iG)_{\mathfrak{c}}}$ where $(\mathrm{d}_iG)_{\mathfrak{c}}$ is obtained from $G$ by fixing all the free cells except for the $i$-th one to the corresponding element of ${\mathfrak{c}}$.


\vspace{10pt}
Consider as a final example the graph $G$ in figure \ref{fig:worked_example_norm} [left] with its specification of in/out vertices and edges.
This defines, choosing $\mathfrak{c} := (c,(a,b))$, a bi-linear map $\bW_G^{\mathfrak{c}}: \bR^{\fd(c)} \times \bR^{\fd(a) \times \fd(b)} \to \bR^{\fd(d)}$ (with the vertex-naming convention of figure \ref{fig:basic-tre--free}).
Given an input sequence $\mathbf{X}_{\mathfrak{c}} := (\mathbf{x} ,W)$, the differential at that point can be written as 
\[
(\mathrm{d}\bW_{G}^{\mathfrak{c}})_{\mathbf{X}_{\mathfrak{c}}} = (\mathrm{d}_{1} \bW_{G}^{\mathfrak{c}})_{\mathbf{X}_{\mathfrak{c}}} +( \mathrm{d}_{2} \bW_{G}^{\mathfrak{c}})_{\mathbf{X}_{\mathfrak{c}}}
= \bW_{(\mathrm{d}_{1} G)_{\mathbf{X}_{\mathfrak{c}}}} + \bW_{(\mathrm{d}_{2} G)_{\mathbf{X}_{\mathfrak{c}}}}
\]
\emph{cf.} figure \ref{fig:worked_example_norm} [middle].


    \begin{figure}[ht]
        \centering
        \input{Figures/worked_example_3}
        \caption{Some operations on Graphs.}
        \label{fig:worked_example_norm}
\end{figure}
Let us, for instance, compute the squared Hilbert-Schmidt norm of $(\mathrm{d}_2\bW_{G}^{\mathfrak{c}})_{\mathbf{X}_{\mathfrak{c}}}$ which in coordinates is given by 
\begin{align*}
    \norm{(\mathrm{d}_2\bW_{G}^{\mathfrak{c}})_{\mathbf{X}_{\mathfrak{c}}}}^2_{HS} =& ~
    Tr\left((\mathrm{d}_2\bW_{G}^{\mathfrak{c}})_{\mathbf{X}_{\mathfrak{c}}}^{\top}(\mathrm{d}_2\bW_{G}^{\mathfrak{c}})_{\mathbf{X}_{\mathfrak{c}}}\right)
    =
    \sum_{\alpha,\beta,\delta} \sprod{\mathbf{e}_{\delta}}{(\mathrm{d}_2\bW_{G}^{\mathfrak{c}})_{\mathbf{X}_{\mathfrak{c}}}[\mathbf{E}_{\alpha,\beta}]}^2.
\end{align*}
This is given by the product graph in figure \ref{fig:worked_example_norm} [right].





% Further, we can also graphically represent the composition of two maps
% $$
% W_G(\mathbf{x}_a,\mathbf{x}_b)=\langle \mathbf{x}_b,\,W_{G'}\mathbf{x}_a\rangle,W_G(\mathbf{x}_a,\mathbf{x}_b)=\langle \mathbf{x}_b,W_{G'}\mathbf{x}_a\rangle.$$ 
% To that end, let $G$


% Given a graph $G$ with two \emph{free} vertices $v,v' \in V(G)$ having the same image $\cv \in V(\cG)$ we can identify these two vertices by contracting the corresponding indices in the tensor. We denote this operation by $\bigwedge_v^{v'}(W_G)$. The result corresponds to the graph obtained by identifying $v$ and $v'$ in a vertex $v\wedge v'$ fixed to have input $\mathbf{1}_{N_{\cv}}$ (see Figure \ref{fig:composition_multi-linear}).\CrisComm{This section 6.1 is still a bit unclear.}

% \begin{figure}[H]
%     \centering
%     \includegraphics[scale = 0.085]{Figures/composition_multi-linear_2.jpeg}
%     \caption{Joining of graphs.}
%     \label{fig:composition_multi-linear}
% \end{figure} 

% A graph $G$ with only two free vertices $a,b$ is a bi-linear map and thus corresponds to a matrix, which we still call $W_G$, as 
% \[
% W_G(v_a,v_b) = \sprod{v_{b}}{W_Gv_{a}} \quad [W_G]_{ij} = W_G(e_i,e_j)
% \]
% In this identification the order $v_a,v_b$ matters, in fact one has as well that 
% \[
% W_G(v_a,v_b) = \sprod{v_{a}}{W_G^{\top}v_{b}}
% \]
% It is important thus, when using this identification between tensor and matrix, to make clear which vertex is the \emph{input} vertex and which one is the \emph{output} vertex. Reversing the roles of the two corresponds to a matrix transposition.

% When the two vertices correspond to the same $\cv \in V(\cG)$ then the matrix is square and we can take its trace. Since the trace is just a contraction we see that $Tr(W_G) = \bigwedge_a^b (W_G)$ (see Figure \ref{fig:Trace_bi-linear}).

% \begin{figure}[H]
%     \centering
%     \includegraphics[scale = 0.085]{Figures/Trace_bi-linear_2.jpeg}
%     \caption{Trace of bi-linear operator is given by another graph operator. }
%     \label{fig:Trace_bi-linear}
% \end{figure} 

% Here it is not necessary to specify the input and output vectors since the trace is invariant under transposition, a fact reflected by the form of the resulting graph.


% To do this, we first  show how the Riesz representation theorem can be used to take different points of view of the same multi-linear map. 

% Consider a graph $G$ with free vertices $V_\cF$ and all edges fixed, which then defines a $|V_\cF|$-linear map  
% \[
%     W_{G}:\prod_{v\in V_\mathcal{F}} \mathbb{C}^{N_v}\to\mathbb{C}.
% \]
% If we partition the set of free vertices into $V_\cF = V_{\cF}^{\mathrm{in}} \bigsqcup  V_\cF^{\mathrm{out}}$ and fix inputs $(\mathbf{x}_v)_{v\in V_{\mathcal{F}}^{\mathrm{in}}}$ for those in $V_\mathcal{F}^{\mathrm{in}}$, then the Riesz representation theorem applied to the map $$W_G((\mathbf{x}_{v})_{v\in V_{\mathcal{F}}^{\mathrm{in}}}, .)$$ yields the existence of a unique vector $\boldsymbol{\Psi}_{\mathrm{in}}\in \bigotimes_{u\in V_{\mathcal{F}}^{\mathrm{out}}} \mathbb{C}^{N_{u}}$
% satisfying 
% \begin{equation}
%     \sprod{\boldsymbol{\Psi}_\mathrm{in}}{\otimes_{u\in V_{\mathcal{F}}^{\mathrm{out}}} \mathbf{y}_{ u}} := W_{G}\left((\mathbf{x}_v)_{v\in V_{\mathcal{F}}^{\mathrm{in}}},(\mathbf{y}_{u})_{ u\in V_{\mathcal{F}}^{\mathrm{out}}}\right).
% \end{equation}
% If we let $\mathcal{G}$ denote the graph $G$ together with a choice of partition $V_\cF = V_{\cF}^{\mathrm{in}} \bigsqcup  V_\cF^{\mathrm{out}}$, then this procedure yields a map
% \[
%  W_{\mathcal{G}}:\prod_{v\in V_\mathcal{R}^{\mathrm{in}}}\mathbb{C}^{N_v}\rightarrow \prod_{u\in V_\mathcal{R}^{\mathrm{out}}}\mathbb{C}^{N_u},\quad(\mathbf{x}_v)_{v\in V_\mathcal{R}^{\mathrm{in}}}\mapsto\boldsymbol{\Phi}_\mathrm{in}.
% \]


% \[
% \bW_{G}:\bigotimes_{v\in V_{\mathcal{F}}^{\mathrm{in}}} \mathbb{R}^{N_v} \to \bigotimes_{u\in V_{\mathcal{F}}^{\mathrm{out}}} \mathbb{R}^{N_{u}}, \quad \otimes_{v\in V_{\mathcal{F}}^{\mathrm{in}}} \mathbf{x}_v \mapsto \bW_{G}[\otimes_{v\in V_{\mathcal{F}}^{\mathrm{in}}} \mathbf{x}_v]
% \]
% where $\bar{W}_{G}[\otimes_{v\in V_{\mathcal{F}}^{\mathrm{in}}} \mathbf{x}_v]$ is the unique vector in $\bigotimes_{u\in V_{\mathcal{F}}^{\mathrm{out}}} \mathbb{C}^{N_{u}}$ such that 
% \begin{equation}
%     \sprod{\bW_{G}[\otimes_{v\in V_{\mathcal{F}}^{\mathrm{in}}} \mathbf{x}_v]}{\otimes_{u\in V_{\mathcal{F}}^{\mathrm{in}}} \mathbf{y}_{ u}} := W_{G}\left((\mathbf{x}_v)_{v\in V_{\mathcal{F}}^{\mathrm{in}}},(\mathbf{y}_{u})_{ u\in V_{\mathcal{F}}^{\mathrm{in}}}\right).
% \end{equation}

% While this may seem convoluted and unmotivated first glance, operations on $M_G$ have the benefit of being particularly simple to describe in terms of the graph $G$. For instance, graphically representing the transpose $M_G^{T}$ is as simple as swapping our previous choice of free vertices, taking $\cF_{\mathrm{in}} = \{b\}, ~  \cF_{\mathrm{out}} = \{a\}$. A matrix product $M_{G_1}M_{G_2}$ will correspond to attaching the graphs $G_1$ and $G_2$ by one of their vertices. This example, among others, is depicted in the figures below. 
% \JadComm{There's something a bit off in the exposition here; having defined product graphs to give us matrix products on a path, why would the reader be impressed by this huge detour which only gives another product at the end? Maybe we should not talk about the matrix representation at all, even in the bilinear case, and only keep things in terms of operators?}

% Note that to avoid clutter, we will omit the specification of $\cF_{\mathrm{in}}, ~  \cF_{\mathrm{out}}$ in our equations, opting instead to make this choice clear in the figures where it will be explicitly shown (\emph{cf.} Figure \ref{fig:Riesz_Graphs}).

% \begin{figure}[!h]
%         \centering
%         \scalebox{0.90}{\input{Figures/Riesz_Graphs}}
%         \caption{Choosing \emph{input} and \emph{output} vertices allows to consider the graph as defining a matrix, or a vector, which is the Riesz representation of its associated linear map.}
%         \label{fig:Riesz_Graphs}
% \end{figure}

% Here we used $W_G$ to denote both the bi-linear map and its matrix representation. Note that the latter isn't canonical here, as it depends on the order of the inputs; switching that order would amount to taking the transpose of that matrix. 

% We note that 
% \begin{example}[Evaluations and Projections]
%     Evaluating an operator $\bW_G$ in some $\mathbf{X}_{c^*}$ for $c^* \in \cF_{\mathrm{in}}$ corresponds to pre-composing it by the map
%     \[
%     \otimes_{ c \in \cF_{\mathrm{in}}\setminus\{c^*\}}  \mathbf{X}_{c}
%     \mapsto \otimes_{ c \in \cF_{\mathrm{in}}}  \mathbf{X}_{c}
%     \]
%     while projecting it by some $\mathbf{Y}_{c'}$ for $c' \in \cF_{\mathrm{out}}$
%     corresponds to post-composing it by the map
%     {
%     \[
%     \otimes_{ c \in \cF_{\mathrm{out}}}  \mathbf{X}_{c}
%     \mapsto 
%     \sprod{\mathbf{X}_{c'}}{\mathbf{Y}_{c'}}_{\bC^{\fd(c)}}
%     \left( \otimes_{ c \in \cF_{\mathrm{out}}\setminus\{c'\}}  \mathbf{X}_{c} \right)
%     \]
%     }
%     Graphically both of these operations correspond to simply fixing respectively the cells $c^*$ and $c'$ to $\mathbf{X}_{c^*}$ and $\mathbf{Y}_{c'}$ (\emph{cf.} figure \ref{fig:Riesz_Graphs} [middle]).
% \end{example}
% \JadComm{Why did we need the inputs to be a sequence and not a set already? and how do we give a canonical ordering of that sequence?}
% \begin{example}[Evaluation] If $G=(G,\mathcal{F}_{\mathrm{out}},\mathcal{F}_\mathrm{in}, (\mathbf{X}_c)_{c\in C\setminus \mathcal{F}})$ is an operator graph and $\mathbf{W}_G$ is its associated map, then the evaluation of $\mathbf{W}_G$ at some $\mathbf{X}_{c_0}$ in its $c_0$-th input slot is given by $\mathbf{W}_{G'}$, where 
% \[  
%     G'=(G,\mathcal{F}_{\mathrm{out}},\mathcal{F}_\mathrm{in}\setminus\{c_0\}, (\mathbf{X}_c)_{c\in C\setminus\mathcal{F}}\cup \{\mathbf{X}_{c_0}\}).
% \]
% This is depicted in figure \ref{fig:fixing} (middle), and corresponds to simply fixing the cell $c_0$ to have input $\mathbf{X}_{c_0}$ by replacing $\circ$ with $\bullet_{\mathbf{X}_{c_0}}$.
% \end{example}
% \begin{example}
    
% \end{example}

==> Sections/ideas.tex <==
Let's take a long term view, maybe it will help streamline notation and ideas.
What construction do we want to have?

We need to work with \emph{simplicial complexes}, that is sequences of simplices
\[
\mathcal{C} := (C_{0}, C_1, \dots, C_n)
\]
where each $C_k$ is composed of directed $k$-simplices whose vertices are in $C_{0}$. One way to do this is to construct first the set of vertices $C_0$, then that of edges $C_1$ as a subset of $C_0 \times C_0$, and so on building $C_{k}$ as a subset of $(C_{0})^{k+1}$.
Each of the \emph{cell} sets $C_k$ will be partitioned as 
\[
C_k = C_k^{\mathrm{free}} \sqcup C_k^{\mathrm{fix}}
\]
in a set of free cells and one of fixed cells, in turn
\[
C_k^{\mathrm{free}} = C_k^{\mathrm{in}} \sqcup C_k^{\mathrm{out}}.
\]

The fixed $k$-cells will be associated to $k+1$-tensors $\mathbb{C}_k = (\mathbf{X}_c ~|~ c \in C_k^{\mathrm{fix}})$ where the coordinates are associated to the $k$-cell's vertices in the correct order.

If $C_k^{\mathrm{free}} = \emptyset$ for all $k$ then we call the simplex a \emph{product simplex} and say that its \emph{product} is the scalar
\[
\mathbf{W}_{\mathcal{C}} := \sum_{\mathbf{i} \in N_{C_0}} \prod_{k=0}^n \prod_{c_k \in C_k} [\mathbf{X}_{c_k}]_{\mathbf{i}|_{c_k}}
\]


There will be a subset ${C}_k^{\cR} \subseteq {C}_k^{\mathrm{fix}}$ of cells for which the corresponding $\mathbf{X}_c$ have iid Gaussian coordinates.
We will need to consider admissible pairings  of $\mathcal{C}$
\[
\phi = \phi_0 \sqcup \cdots \sqcup \phi_n
\]
where each $\phi_k$ is an admissible pairing of ${C}_k^{\cR}$.
Any such admissible pairing $\phi$ will induce a \emph{partition} $\Phi$ of $\mathcal{C}$
\[
\Phi = \Phi_0 \sqcup \cdots \sqcup \Phi_n
\]
defined by first grouping together all the vertices of the paired cells in $\phi$, then the edges with vertices in the same $\pi_0 \in \Phi_0$, and so on.

This defines a new complex $\mathcal{C}(\Phi)$ where $C(\Phi)_k \simeq \Phi_k$, this bijection defines a surjective map $C_k \twoheadrightarrow C(\Phi)_k$, which we still call $\Phi$, which sends a $k$-cell $c_k$ to the $k$-cell $\Phi(c_k) \in C(\Phi)_k$ corresponding to the $c_k \in \pi_k \in \Phi_k$.

If $C$ was a product graph then $\mathcal{C}(\Phi)$ is one as well where 
\[
\mathbb{C}(\Phi)_k = \{ \odot_{c \in \pi_k} \mathbf{X}_c ~|~ \pi_k \in \Phi_k\}
\]
so that its product becomes 
\[
\sum_{\mathbf{i} \in N_{\Phi_0}} \prod_{k=0}^n \prod_{\pi_k \in \Phi_k} \prod_{c \in \pi_k}
[\mathbf{X}_{c}]_{\mathbf{i}|_{\pi_k}}
=
\sum_{\mathbf{i} \in N_{\Phi_0}} \prod_{k=0}^n \prod_{c_k \in C_k}
[\mathbf{X}_{c_k}]_{\mathbf{i}|_{\Phi(c_k)}}
\]
which can be written as 
\[
\sum_{\mathbf{i} \in N_{C_0}} \delta_{\mathbf{i}|_{\Phi_0}} 
\prod_{k=0}^n \prod_{c_k \in C_k}
[\mathbf{X}_{c_k}]_{\mathbf{i}|_{c_k}}
\]
where
\[
\delta_{\mathbf{i}|_{\Phi_0}} = \prod_{\pi_0 \in \Phi_0} \mathbf{1}(\forall v,v' \in \pi_0. ~ i_v = i_{v'})
\]

\section{Some Graph Equivalences}

\begin{figure}[ht]
    \centering
    \scalebox{.8}{\input{Figures/graph_bonanza}}
    \caption{In the bottom equivalence $A = \sum_i \sigma_i \mathbf{u}_i \mathbf{v}_i^{\top}$ is the SVD.}
    \label{fig:graph_bonanza}
\end{figure}


==> Sections/informal_extensions.tex <==
 In order to best illustrate our approach, we chose to restrict all of our results to the simple case of feed-forward networks with polynomial activations and no biases. This leaves room for many possible extensions, and we discuss a few of these informally below. 

\subsection{Random biases}
The $\Phi_L$ that we have considered
are compositions of linear maps $W_\ell$ and component-wise non-linear activations $\varphi_{\ell}$. Typically one considers affine maps $W_{\ell}(\cdot) + b_{\ell}$ instead, and takes the $b_\ell$ to be randomly initialised with Gaussian entries as well.

 The arguments here can be adapted to this case by allowing vertices to be fixed to these $b_{\ell}$, and considering pairings of the vertices as well (resulting in $\sigma_b^2 \mathbf{1}$ in $\bW_{G_\phi}$), as shown in Figure \ref{fig:bias_tree}.

\begin{figure}[h!]
    \centering
    \input{Figures/bias_tree}
    \caption{Example of a tree arising in the expansion of a neural network with biases.}
    \label{fig:bias_tree}
\end{figure}

\subsection{Residual networks and other neural network architectures} 
\label{subsec:other_arch}
We briefly discuss how our theory can be extended to more complex neural network architectures, beginning with the simplest example: \emph{residual networks}. 

Recall that for the feed-forward networks considered in this paper, the network's input is represented by fixing some leaf vertices' input to $\mathbf{x}$. 
In a residual network, a new layer $Z_{L+1}$ is obtained by adding the output $Z_L$ of the previous layer to the output of a feed-forward network $\Phi$ taking $Z_L$ as input.
Consequently, the trees that will arise in the expansion of $Z_{L+1}$ are formed by grafting the trees from the expansion of $Z_L$ onto the leaves of the trees for $\Phi(\bx)$. The theory developed here thus extends to discrete residual networks with minimal modifications.

 For continuous networks, the graphs arising in the expansion can be arbitrarily deep, there are infinitely many of them. Some care is therefore needed to ensure that the expansions are well-defined, namely that they converge. 


More complex architectures can be studied by considering \emph{simplicial complexes} instead of graphs. 
For instance, for architectures like convolutional neural networks, generic tensors must be considered in addition to matrices and vectors. 
Just as the former correspond to edges ($1$-simplices) and the latter to vertices ($0$-simplices), an $n+1$-tensor will correspond to an $n$-simplex. The resulting  network expansion will then be over simplicial complexes, typically exhibiting a tree-like recursive structure. 
The theory then requires pairing $n$-tensors with $n$-tensors and counting the number of vertices in the resulting simplices.


\subsection{Non-polynomial activations}

A restriction we have imposed is the use of polynomial activations $\varphi_{\ell}$.
This choice allowed us to ignore questions of convergence (e.g. for the tree expansion in Theorem \ref{thm:tree_exp}) given that the sums being considered are always finite. Polynomials being dense in Gaussian Sobolev spaces, we expect an extension of our results to commonly used, non-polynomial activations (e.g. Sigmoid, ReLU) to be possible through a density argument, and present some numerical evidence for this in Appendix \ref{app:numerics}.


% \subsection{Spectrum of the Hessian matrix} A rigorous understanding of the spectrum of the Hessian matrix under training would shed light on important aspects of the training dynamics, particularly on its speed and stability as argued in \cite{noci2024learningratestransferreconciling, orvieto2021vanishingcurvaturepoweradaptive}.
% We expect to be able to study the empirical spectral distribution of the Hessian matrix of $\Phi_L$ using arguments similar to those in Sections \ref{sec:jacobian} and \ref{sec:NTK}, but anticipate the combinatorics that would ensue to be more involved.


